SurfaceNet+: An End-to-end 3D Neural Network for Very Sparse Multi-view Stereopsis

Multi-view stereopsis (MVS) tries to recover the 3D model from 2D images. As the observations become sparser, the significant 3D information loss makes the MVS problem more challenging. Instead of only focusing on densely sampled conditions, we investigate sparse-MVS with large baseline angles since the sparser sensation is more practical and more cost-efficient. By investigating various observation sparsities, we show that the classical depth-fusion pipeline becomes powerless for the case with a larger baseline angle that worsens the photo-consistency check. As another line of the solution, we present SurfaceNet+, a volumetric method to handle the 'incompleteness' and the 'inaccuracy' problems induced by a very sparse MVS setup. Specifically, the former problem is handled by a novel volume-wise view selection approach. It owns superiority in selecting valid views while discarding invalid occluded views by considering the geometric prior. Furthermore, the latter problem is handled via a multi-scale strategy that consequently refines the recovered geometry around the region with the repeating pattern. The experiments demonstrate the tremendous performance gap between SurfaceNet+ and state-of-the-art methods in terms of precision and recall. Under the extreme sparse-MVS settings in two datasets, where existing methods can only return very few points, SurfaceNet+ still works as well as in the dense MVS setting. The benchmark and the implementation are publicly available at https://github.com/mjiUST/SurfaceNet-plus.

==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/


This package contains the IEEE Computer Society subset of the full IEEEtran
package and is intended for use with IEEE Computer Society publications.
The included version of the IEEEtran_HOWTO.pdf has been specially formatted
in IEEE Computer Society (compsoc) journal mode.


For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for a IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf_compsoc.tex, bare_jrnl_compsoc.tex.
***************************************************************************


==> sections/_x_-SurfaceNet_overview.tex <==
\subsection{SurfaceNet}\label{SurfaceNet_overview}


SurfaceNet first handle the problem of reconstruction from two views. Given two images ($I_i$,$I_j$),its corresponding camera views ($v_i$,$v_j$) and a 3D tensor $C$ of the voxelized scene ,SurfaceNet proposed an end-to-end learning framework to reconstruct the 3D surface in $C$ by estimating for each voxel $x\in C$ if it is on the surface or not. First Two images $I_i$ and $I_j$ are converted to a 3D voxel representation called \textit{colored voxel cube} (CVC) that encodes the camera parameters implicitly in it.The detailed explanation are shown in Fig~\ref{fig:cvc_demo}.
\begin{figure}[h] % t/b/h: put the figure at the top / bottom / here
\centering
    \includegraphics[width=0.8\linewidth]{figures/method/cvc_demo} % scale=1 / width=0.8\linewidth\textwidth
    \caption{Illustration of Colored Voxel Cubes (CVC). Given a view $v$(left), we convert the image $I_v$ into a 3D colored cube $I^C_v$ by projecting each pixel $I_vp$ to all the voxel $x \in C$ and storing the RGB values $i_x$ for each voxel respectively(middle and right).The camera parameters are encoded implicitly with CVC.}
    \label{fig:cvc_demo}
\end{figure}

After getting two colored voxel cubes ($C_i$,$C_j$),a U-Net structured fully 3D convolutional network was taken to predict the confidence $p_x \in (0,1)$ on each voxel $x \in C$, which indicates if a voxel is on the surface or not.Since the network is fully convolutional, the size of the CVC cubes can be adaptive and the output is always the same size as the CVC cubes.
SurfaceNet used a class-balanced cross-entropy function as loss for training and ray pooling operation to convert the probabilities into a surface during inference stage.

To generalize to multiple views, SurfaceNet selected a subset of view pairs $(v_i,v_j)$ from all available views  $v_1, \ldots, v_V$ .For each image $I_{v_i}$ and $I_{v_j}$ , SurfaceNet predicts $p^{(v_i,v_j)}_x$, \ie the confidence that a voxel $x$ is on the surface,then combined together by taking the weighted average of the predictions $p^{(v_i,v_j)}_x$.The relative weights for each view pair are then given by this way: A $64\times64$ patch was cropped around the projected center voxel of $C$ , then a feature embedding $e(C,I_{v_i})$ was generated by a triplet network~\cite{schroff2015facenet} from the patch to a compact 128D Euclidean space . Combined with the relation of the two viewpoints $v_i$ and $v_j$, the relative weights can be written by:
\begin{equation} \label{eq:relativeImportance}
 w_C^{(v_i,v_j)} = r\left(\theta_C^{(v_i,v_j)}, e(C,I_{v_i})^T, e(C,I_{v_j})^T \right)
\end{equation}
 $\theta_C^{(v_i,v_j)}$ is the angle between the projection rays from the center voxel of $C$ to the two viewpoints $v_i$ and $v_j$ and  $r(\cdot)$ is a fully connected neural network.
The weighted average of the predicted surface probabilities $p_x^{(v_i, v_j)}$ is 		
\begin{equation} \label{eq:fusion}
    p_x = \frac{\sum_{(v_i,v_j) \in \bm{V}_C}w_C^{(v_i,v_j)} p_x^{(v_i, v_j)}}
        {\sum_{(v_i,v_j) \in \bm{V}_C}w_C^{(v_i,v_j)}}
\end{equation}
where $\bm{V}_c$ denotes the set of selected view pairs. Since it is unnecessary to take all view pairs into account, we select only $N_v$ view pairs, which have the highest weight $w_C^{(v_i,v_j)}$. 



==> sections/_x_-conclusion.tex <==
%=========================================================================
\section{Conclusion}


In this work, we presented a faster deep reconstruction strategy for sparse view stereo reconstruction. Instead of reconstructing the scene at the given resolution, we predict different scales of shape from coarse to fine.We sample cubes around the coarse predicted point cloud and perform occlusion detection to produce better view pairs. Experiments show that with the proposed coarse-to-fine and occlusion detection mechanism, SurfaceNet+ outperforms the state-of-art method and has steady performance under very sparse scenes.  Also, SurfaceNet+ is ten times faster than SurfaceNet and has a very efficient reconstruction strategy.

==> sections/_x_-discussion.tex <==

%- - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - -
\subsection{discussion and future work}

\textbf{potentials}
1. such 3D network design can be valuable for other 3D applications, such as point cloud denoising and holes filling.
2. the learned 3D kernels could be used to replace the hand-crafted 3D features and descriptors. 
    Consequently, it can be used for the applications like point cloud registration and semantic labeling.
\par

\textbf{future work}
1. speedup using sparse representation of the surface model. (sparseCNN, octreeCNN, ...)
2. combine with semantic information:
    a. combine with the 2D image semantic labels by expanding into the color channels in the colored voxel cube;
    b. directly supervise and infer dense 3D semantic labels.
\par 
% % about the new method's error pattern
% The network learns some surface structure information, which is relatively higher level than voxel level photo consistency method.
% So that it can be more robust to not-too-large pure color regions, for example in the model12 middle part of letters other methods will have small holes.
% 
% problem: repeating pattern and pure color region.
% 
% Interestingly, we haven't use 'pool along the ray' (?) condition yet. 
% The reason we didn't use the postprocessing like hole filling / outlayer rejection is that we want show our new method alone can be competitive to the state of the art methods, some of which have several postprocessing stages.
% 
% 


==> sections/_x_-formatting.tex <==
\section{Formatting your paper}

All text must be in a two-column format. The total allowable width of the
text area is $6\frac78$ inches (17.5 cm) wide by $8\frac78$ inches (22.54
cm) high. Columns are to be $3\frac14$ inches (8.25 cm) wide, with a
$\frac{5}{16}$ inch (0.8 cm) space between them. The main title (on the
first page) should begin 1.0 inch (2.54 cm) from the top edge of the
page. The second and following pages should begin 1.0 inch (2.54 cm) from
the top edge. On all pages, the bottom margin should be 1-1/8 inches (2.86
cm) from the bottom edge of the page for $8.5 \times 11$-inch paper; for A4
paper, approximately 1-5/8 inches (4.13 cm) from the bottom edge of the
page.

%-------------------------------------------------------------------------
\subsection{Margins and page numbering}

All printed material, including text, illustrations, and charts, must be kept
within a print area 6-7/8 inches (17.5 cm) wide by 8-7/8 inches (22.54 cm)
high.



%-------------------------------------------------------------------------
\subsection{Type-style and fonts}

Wherever Times is specified, Times Roman may also be used. If neither is
available on your word processor, please use the font closest in
appearance to Times to which you have access.

MAIN TITLE. Center the title 1-3/8 inches (3.49 cm) from the top edge of
the first page. The title should be in Times 14-point, boldface type.
Capitalize the first letter of nouns, pronouns, verbs, adjectives, and
adverbs; do not capitalize articles, coordinate conjunctions, or
prepositions (unless the title begins with such a word). Leave two blank
lines after the title.

AUTHOR NAME(s) and AFFILIATION(s) are to be centered beneath the title
and printed in Times 12-point, non-boldface type. This information is to
be followed by two blank lines.

The ABSTRACT and MAIN TEXT are to be in a two-column format.

MAIN TEXT. Type main text in 10-point Times, single-spaced. Do NOT use
double-spacing. All paragraphs should be indented 1 pica (approx. 1/6
inch or 0.422 cm). Make sure your text is fully justified---that is,
flush left and flush right. Please do not place any additional blank
lines between paragraphs.

Figure and table captions should be 9-point Roman type as in
Figures~\ref{fig:onecol} and~\ref{fig:short}.  Short captions should be centred.

\noindent Callouts should be 9-point Helvetica, non-boldface type.
Initially capitalize only the first word of section titles and first-,
second-, and third-order headings.

FIRST-ORDER HEADINGS. (For example, {\large \bf 1. Introduction})
should be Times 12-point boldface, initially capitalized, flush left,
with one blank line before, and one blank line after.

SECOND-ORDER HEADINGS. (For example, { \bf 1.1. Database elements})
should be Times 11-point boldface, initially capitalized, flush left,
with one blank line before, and one after. If you require a third-order
heading (we discourage it), use 10-point Times, boldface, initially
capitalized, flush left, preceded by one blank line, followed by a period
and your text on the same line.

%-------------------------------------------------------------------------
\subsection{Footnotes}

Please use footnotes\footnote {This is what a footnote looks like.  It
often distracts the reader from the main flow of the argument.} sparingly.
Indeed, try to avoid footnotes altogether and include necessary peripheral
observations in
the text (within parentheses, if you prefer, as in this sentence).  If you
wish to use a footnote, place it at the bottom of the column on the page on
which it is referenced. Use Times 8-point type, single-spaced.


%-------------------------------------------------------------------------
\subsection{References}

List and number all bibliographical references in 9-point Times,
single-spaced, at the end of your paper. When referenced in the text,
enclose the citation number in square brackets, for
example~\cite{Authors14}.  Where appropriate, include the name(s) of
editors of referenced books.

\begin{table}
\begin{center}
\begin{tabular}{|l|c|}
\hline
Method & Frobnability \\
\hline\hline
Theirs & Frumpy \\
Yours & Frobbly \\
Ours & Makes one's heart Frob\\
\hline
\end{tabular}
\end{center}
\caption{Results.   Ours is better.}
\end{table}

%-------------------------------------------------------------------------
\subsection{Illustrations, graphs, and photographs}

All graphics should be centered.  Please ensure that any point you wish to
make is resolvable in a printed copy of the paper.  Resize fonts in figures
to match the font in the body text, and choose line widths which render
effectively in print.  Many readers (and reviewers), even of an electronic
copy, will choose to print your paper in order to read it.  You cannot
insist that they do otherwise, and therefore must not assume that they can
zoom in to see tiny details on a graphic.

When placing figures in \LaTeX, it's almost always best to use
\verb+\includegraphics+, and to specify the  figure width as a multiple of
the line width as in the example below
{\small\begin{verbatim}
   \usepackage[dvips]{graphicx} ...
   \includegraphics[width=0.8\linewidth]
                   {myfile.eps}
\end{verbatim}
}


%-------------------------------------------------------------------------
\subsection{Color}

Please refer to the author guidelines on the CVPR 2017 web page for a discussion
of the use of color in your document.



==> sections/_x_-fusion.tex <==
\section{Multi-View Stereopsis}\label{multiViewFusion}
So far we have described training and inference with SurfaceNet if only two views are available. We now describe how it can be trained and used for multi-view stereopsis.

\subsection{Inference}\label{multiViewFusion:inf}
If multiple views $v_1, \ldots, v_V$ are available, we select a subset of view pairs $(v_i,v_j)$ and compute for a cube $C$ and each selected view $v$ the CVC cube $I^C_{v}$. We will discuss at the end of the section how the view pairs are selected.

For each view pair $(v_i,v_j)$, SurfaceNet predicts $p^{(v_i,v_j)}_x$, \ie the confidence that a voxel $x$ is on the surface. The predictions of all view pairs can be combined by taking the average of the predictions $p^{(v_i,v_j)}_x$ for each voxel. However, the view pairs should not be treated equally since the reconstruction accuracy varies among the view pairs. In general, the accuracy depends on the viewpoint difference of the two views and the presence of occlusions. 

To further identify occlusions between two views $v_i$ and $v_j$, we crop a $64\times64$ patch around the projected center voxel of $C$ for each image $I_{v_i}$ and $I_{v_j}$. 
To compare the similarity of the two patches, we train a triplet network~\cite{schroff2015facenet} that learns a mapping $e(\cdot)$ from images to a compact 128D Euclidean space %, say $\mathbb{R}^{128}$, 
    where distances directly correspond to a measure of image similarity. 
The dissimilarity of the two patches is then given by
\begin{equation} \label{eq:similarity}
    d_C^{(v_i,v_j)} = \lVert e(C,I_{v_i})-e(C,I_{v_j}) \rVert_2,
\end{equation}
where $e(C,I_{v_i})$ denotes the feature embedding provided by the triplet network for the patch from image $I_{v_i}$. 
This measurement can be combined by the relation of the two viewpoints $v_i$ and $v_j$, which is measured by the angle between the projection rays of the center voxel of $C$, which is denoted by $\theta_C^{(v_i,v_j)}$.
We use a 2-layer fully connected neural network $r(\cdot)$, that has 100 hidden neurons with sigmoid activation function and one linear output neuron followed by a softmax layer. The relative weights for each view pair are then given by
\begin{equation} \label{eq:relativeImportance}
 w_C^{(v_i,v_j)} = r\left(\theta_C^{(v_i,v_j)}, d_C^{(v_i,v_j)}, e(C,I_{v_i})^T, e(C,I_{v_j})^T \right)
\end{equation}
and the weighted average of the predicted surface probabilities $p_x^{(v_i, v_j)}$ by 		
\begin{equation} \label{eq:fusion}
    p_x = \frac{\sum_{(v_i,v_j) \in \bm{V}_C}w_C^{(v_i,v_j)} p_x^{(v_i, v_j)}}
        {\sum_{(v_i,v_j) \in \bm{V}_C}w_C^{(v_i,v_j)}}
\end{equation}
where $\bm{V}_c$ denotes the set of selected view pairs. Since it is unnecessary to take all view pairs into account, we select only $N_v$ view pairs, which have the highest weight $w_C^{(v_i,v_j)}$. In Section \ref{experiments}, we evaluate the impact of $N_v$.

The binarization and thinning are performed as in Section \ref{inference}, \ie  a voxel $x$ is converted into a surface voxel if at least $\gamma=80\%$ of all views vote for it during ray pooling and $p_x > \tau$.
The effects of $\gamma$ and $\tau$ are further elaborated in Section \ref{experiments}.

\subsection{Training}
The SurfaceNet can be trained together with the averaging of multiple view pairs~(\ref{eq:fusion}). We select for each cube $C$, $N_v^{train}$ random view pairs and the loss is computed after the averaging of all view pairs. We use $N_v^{train}=6$ as a trade-off since larger values increase the memory for each sampled cube $C$ and thus require to reduce the batch size for training due to limited GPU memory. Note that for inference, $N_v$ can be larger or smaller than $N_v^{train}$.

In order to train the triplet network for the dissimilarity measurement $d_C^{(v_i,v_j)}$~(\ref{eq:similarity}), we sample cubes $C$ and three random views where the surface is not occluded. The corresponding patches obtained by projecting the center of the cube onto the first two views serve as a positive pair. The negative patch is obtained by randomly shifting the patch of the third view by at least a quarter of the patch size. While the first two views are different, the third view can be the same as one of the other two views.
At the same time, we use data augmentation by varying illumination or adding noise, rotation, scale, and translation.
%Note that the translation variance is not considered for the negative view, since image translation will break the link between the 3D point and the view patch.
After SurfaceNet and the triplet network are trained, we finally learn the shallow network $r(\cdot)$ (\ref{eq:relativeImportance}). 

%Finally the shallow network $r(\cdot)$ (\ref{eq:relativeImportance}) can be updated by keeping the learned models of SurfaceNet and the triplet net.



%
%% fuse multiple view pairs' prediction
%In order to get accurate result, we fuse probability cubes $c^p(v_i,v_j)$
    %from multiple view pairs by weighted average.
%The weight is interpreted as the relative importance of each view pair.
%
%\textbf{Relative importance:}
%% why define relative importance
%Even though each view pair can predict one version of the surface segment,
    %different view pair candidates should not be teated equally in the fusion procedure.
%$w(c, v_i, v_j)$ is defined as the relative importance of
    %the predicted surface in the cube $c$ based on the view pair $(v_i,v_j)$.
%The reason why it is called relative importance is that a single
    %$w(c, v_i, v_j)$ value is meaningless until compared with another
    %$w(c, v_{i'}, v_{j'})$ to distinguish which view pair can contribute more
    %for the final prediction.
%\par
%
%% how to calculate
%As widely known that the baseline between a pair of view is crutial
    %to determine the accuracy of the stereo matching.
%In a certain range, the larger the baseline is, the higher the matching accuracy will be.
%Beyond the certain range it also happens that the matching accuracy drops
    %as the baseline keeps increasing, which is caused by complex geometric strucuture or severe occlusion of the scene.
%Therefore, the relative importance is not only influenced by the baseline.
%The occlusion and the complexity of the 3D surface should also be considered.
%We train another triplet network like \cite{schroff2015facenet} to learn an embedding
    %$e(\cdot) \in \mathbb{R}^d$ mapping an image patch $P(c,v_i)$ into a d-dimentional Euclidean space.
%One the manifold, the shorter Euclidean distance $d(c,v_i,v_j)$ between the embeddings of an image patch pair
    %is understood as a higher probability that the center voxel $\dot{x}$ of $c$ is potentially on the model surface.
%If any views in $\{v_i, v_j\}$ are occluded to observe the center voxel $\dot{x}$ of $c$,
    %generally $d(c,v_i,v_j)$ is quite large to be distinguishable.
%So that $d(c,v_i,v_j)$ could be treated as another measurement to predict the relative importance term.
%Additionally, the more texture the image patch has, the more accurate the reconstruction result will be,
    %the higher the relative value should be.
%So we add more high level discriptions of the patches to determine $w(c,v_i,v_j)$.
%\par
%
%So we define the relative importance as the combination of the baseline,
    %which is proportional to the view angle difference $\theta(c,v_i,v_j)$,
    %and extracted features of the image patches $P(c,v_i),P(c,v_j)$:
%\begin{equation} \label{eq:similarity}
    %d(c,v_i,v_j) = \lVert e(P(c,v_i))-e(P(c,v_j)) \rVert_2
%\end{equation}
%\begin{equation} \label{eq:relativeImportance}
    %% w(c,v_i,v_j) = \sigma(w_1*d(c,v_i,v_j) + w_2*\theta(c,v_i,v_j) + b)
    %\begin{split}
        %w(c,v_i,v_j) &= r([\theta(c,v_i,v_j), d(c,v_i,v_j), \\
                     %&e(P(c,v_i))^T, e(P(c,v_j))^T]^T)
    %\end{split}
%\end{equation}
    %where $r(\cdot)$ is simply a multi-layer perception to balance the several features.
    %The training process of $d(\cdot)$ and $r(\cdot)$ is described in Sec.\ref{train}.
%\par
%% The substitution of the function $e(\cdot)$ could be feature extracters,
%%     such as SIFT \cite{lowe2004distinctive} and LIFT \cite{yi2016lift},
%%     and some trained feature embeddings, like the DeepFace \cite{schroff2015facenet}.
%
%\textbf{Fusion:}
%After defining the relative importance of each view pair,
    %we can fuse multiple surface predictions into one by weighted average:
%\begin{equation} \label{eq:fusion}
    %\hat{c}^p = \frac{\sum_{(v_i,v_j) \in \bm{V}_c}{w(c, v_i, v_j) * c^p(v_i, v_j)}}
        %{\sum_{(v_i,v_j) \in \bm{V}_c}{w(c, v_i, v_j)}}
%\end{equation}
%where $\bm{V}_c = \bm{\bar{V}}$, $\bm{\bar{V}}$ is a set of all possible view pairs.
%\par




==> sections/_x_-implementation.tex <==
\section{Implementation Details}\label{implementation}\label{adaptivethres}
%= = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = =
As described in Section~\ref{inference}, the scene volume needs to be divided into cubes due to limitations of the GPU memory. However, it is only necessary to process cubes that are very likely to contain surface voxels. As an approximate measure, we apply logistic regression to the distance vector $d_C^{(v_i,v_j)}$~(\ref{eq:similarity}) for each view pair, which predicts if the patches of both views are similar. If for less than $N_{min}$ of the view pairs the predicted similarity probability is greater than or equal to $0.5$, we reject the cube. 

% we compute $\sigma(d_C^{(v_i,v_j)})$~(\ref{eq:similarity}) for each view pair, where $\sigma(\cdot)$ is a sigmoid function that maps the values to $[0,1]$. If for less than $N_{min}$ of the view pairs $\sigma(d_C^{(v_i,v_j)})\geq 0.5$, we reject the cube. 

Instead of using a single threshold $\tau$ for binarization, one can also adapt the threshold for each cube $C$ based on its neighboring cubes $\mathcal{N}(C)$. The approach is iterated and we initialize $\tau_C$ by $0.5$ for each cube $C$. We optimize \mbox{$\tau_C \in [0.5,1)$} by minimizing the energy 
\begin{equation} \label{eq:E}
    E(\tau_C) = \sum_{C' \in \mathcal{N}(C)}{\psi\left(S^C(\tau_C), S^{C'}(\tau_{C'})\right)}, 
\end{equation}     
where $S^C(\tau_C)$ denotes the estimated surface in cube $C$ after binarization with threshold $\tau_C$.  

For the binary term $\psi$, we use 
\begin{equation}\label{eq:psi}
    \psi(S^C, S^{C'}) = \sum_{x \in C\cap C'} (1-s_x) s'_x + s_x (1-s'_x) - \beta s_x s'_x .
\end{equation}
The first two terms penalize if $S^C$ and $S^{C'}$ disagree in the overlapping region, which can be easily achieved by setting the threshold $\tau$ very high such that the overlapping region contains only very few surface voxels. The last term therefore aims to maximize the surface voxels that are shared among the cubes.       
\par
We used the \textit{Lasagne} Library \cite{lasagne} to implement the network structure. The code and the trained model are publically available.\footnote{\url{https://github.com/mjiUST/SurfaceNet}}
% lasagne
% We used the public available \textit{Lasagne} Library \cite{lasagne} to implement the network structure.
% The training process takes roughly 5 days using a Nvidia TITAN X GPU.
% \par


 

%\subsection{speed up}
%Because of the nature that the model surface sparsely occupies the 3D space,
    %only small amount of the voxel cubes need to be processed to reconstruct the entire scene in a bounded 3D space.
%To further speed up, for each voxel cube $c$ only few view pairs' predictions are enough to generate $\hat{c}^p$.
%\par

%\textbf{Sparse initialization:}
%% regular grid 
%Previously we defined the surfaceNet to predict surface segment in each cube $c \in \bm{C}_{\bm{I}}$.
%In order to speed up, we only consider a small set of voxel cubes 
    %$\bm{C} \subseteq \bm{C}_{\bm{I}}$ nearby the model surface,
%A filter algorithm is designed based on the previously defined $d(c,v_i,v_j)$ that can describe
    %the probability the view patches framing at a same piece of model surface
    %through a logistic regressor $l(\cdot)$, the training of which is discussed in Subsec.\ref{implementation}.
%% define \bm{V}_c
%For each voxel cube $c$, we have a set of view pairs $\bm{V}_c = \bm{\hat{V}}_c$ agreeing that the cube intersects with a piece of surface:
%\begin{equation} \label{eq:viewPairSet}
    %\begin{split} 
        %\bm{\hat{V}}_c &= \{(v_i,v_j)|  v_i,v_j \in \bm{v}, v_i \neq v_j, c \in \bm{C}_{\bm{I}},\\ 
                      %& l(d(c,v_i,v_j)) >= 0.5\} 
    %\end{split}
%\end{equation}
%Finally, the most obvious noisy voxel cubes with less than $N_{min}$ view pairs in $\bm{V}_c$ are filtered out.
%\begin{equation} \label{eq:sparseInit}
    %\bm{C} = \{c|c \in \bm{C}_{\bm{I}}, \left | \bm{\hat{V}}_c \right | >= N_{min}\}
%\end{equation}
%\par

%% use SfM to replace? No
%Ones may wonder whether the result of structure from motion (SfM) can replace the above method.
%The answer is no, as the SfM only results in some sparse 3D key points.
%In the contrary, we prefer the potiential voxel cubes covering the entire model surface.
%\par

%
%\textbf{View pairs selection:} 
%For each voxel cube $c$, there could be as many as $|\bm{\hat{V}_c}| <= |\bm{\bar{V}}|$ 
    %potentially useful view pairs.
%If all of them are considered during fusion,
    %it also be extremely computationally expensive.
%Eventually we only consider few view pairs to reconstruct each surface segment.
%\par
%
%% trivial ways to select view pairs
%There are several ways to select view pairs.
%One trivial way is to choose the view pairs whose baselines are within a certain range.
%As previously discussed, because of the severe occlusion or the complex 3D structure
    %only the baseline information is not enough to compare the potentials of different view pairs.
%Alternatively, some hand-crafted features regarding to the baseline and the view pair's image patches
    %can be designed. 
%However, this is time consuming and not robust enough.
%\par
%
%% our way to select view pairs
%Note that the similar concept is already defined in Sec.\cite{multiViewFusion} the surface fusion procedure
    %as the relative importance $w(c, v_i, v_j)$,
    %indicating how much relative information a view patch pair can offer. 
%We only select $N_v$ view pairs with the highest relative important scores.
%The ideal case is to choose the minimum number of view pairs $N_v=|\bm{\dot{V}}_c|$
    %and to predict the surface as accurate as possible.
%In section \ref{experiments} we will discuss how to choose $N_v$.
%\par

%= = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = =
%\subsection{refinement}
%\textbf{RayPooling:}\label{raypooling}
%With the change of the threshold $\bar{t}_c$, the thickness of the reconstructed surface is get effected.
%In order to reduce the effect from the threshold to the surface thickness, a pooling operation, called rayPooling, is introduced.
%\par
   %
%For a view $v$ and a probability cube $\hat{c}^p$, only one voxel with the max probability value in the set of voxels $\{x^p\}$
    %mapped to the same pixel $p(v,x)$, will be labeled to $1$.
%After loop through $n_v$ views, we only reserve the voxels, whoes accumulated label values larger than $0.8*n_n$.
%
%\textbf{Adaptive threshold:}\label{adaptivethres}
%% why adaptive thresholding
%If the assemblage of the predicted surface segments in each voxel cube 
    %is trivially done by an universial threshold $\bar{t}_c$ in $g(c^p, \bar{t}_c)$ for every $c\in\bm{C}$, 
    %there will be too much noisy surface sugments or the ones with large holes.
%That because the occupancy probability in $c^p$ is only meaningful to distinguish different voxels in one cube
    %and make no sense to compare the voxels across different voxel cubes.
%Therefore, each $c$ needs to find its own $\bar{t}_c$.
%\par
%
%In order to determine $\bar{t}_{c_i}$ for any $c_i$, the neighbouring voxel cubes $c_j^p$ can be considered,
    %where $c_j\in\bm{N_{c_i}}$ represents one of the neighbouring voxel cubes of $c_i$.
%% modeling
%So that inter-volume assemblage procedure can be considered as a simple optimization problem 
    %modeling the interaction between the adjacent surface fragment.
%The optimisation assigns a threshold $\bar{t}_{c_i}$ to each probability cube $\hat{c}_i^p$.
%The cost function to be minimized only consists of pairwise interactins over 
    %first order cliques on the graph constructed upon notes in $\bm{C}$.
%The cost of a threshold $\bar{t}=\{ \bar{t}_i \}$ is expressed as
%\begin{equation} \label{eq:E}
    %E(\bm{\bar{t}}) = \sum_{(c_i,c_j)}{\psi(c_i^s, c_j^s)} 
%\end{equation}
    %where $(c_i,c_j)$ denote neighbouring cubes, $c_j\in\bm{N_{c_i}}$, 
    %$\psi(\cdot,\cdot)$ represents the pairwise interactions function and 
    %$c^s$ is got by thresholding $\hat{c}^p$ using $\bar{t}$.
%\par
%
%Recall that the surface fragment $c^s$ represents empty or occupied voxel using $0$ or $1$.
%% XOR term
%To filter out the noisy surface segments which is floating around and has no connection with other surface,
    %we penalize the dissimilarity between $(c_i^s,c_j^s)$ using $g_{XOR}(c_i^s, c_j^s)$.
%$g_{XOR}(\cdot,\cdot)$ considers the overlapping region of the inputs,
    %computes the XOR operation of each overlapping voxel pair before sum them up.
%% AND term
%Similarly term $g_{AND}(\cdot,\cdot)$ is defined to encourage the continuity of the neighbouring surface fragments
    %by the AND operation.
%% \psi(.,.) function
%Using a user defined weight $\beta$ to balance these two terms, the pairwise interaction function is described as
%\begin{equation}\label{eq:psi}
    %\psi(c_i^s, c_j^s) = g_{XOR}(c_i^s, c_j^s) - \beta * g_{AND}(c_i^s, c_j^s)
%\end{equation}
%\par
%
%% unexpected local minimal
%Note that there is a local minimum of $E(\bm{\bar{t}})$ in the case $\bm{\bar{t}}=\bm{1}$,
    %where after thresholding every voxel cube is empty.
%In order to avoid this local minima trap, we define a certain range for $\bar{t} \in [0.5, \bar{t}_{max}]$. 
%$\bar{t}_{max}<1$ is defined as a threshold which leads to very confident surface fragments $c^s$.
%The optimal thresholds $\bm{\hat{t}}$ is determined as
%\begin{equation}\label{eq:opt_t}
    %\bm{\hat{t}} = \arg \underset{(\bm{\bar{t}})}{min} E(\bm{\bar{t}}) 
                %\;\;\; s.t. \; \bar{t} \in [0.5, \bar{t}_{max}]
%\end{equation}
%A numerical solution of $\bm{\hat{t}}$ is founded under a initial condition 
    %$\bar{t}_{init} = 0.5$ simply using gradient descent.
%


==> sections/_x_-overview.tex <==
\section{Overview}


% \begin{figure*}[t]
% \centering
%     % Prof. Gall: if show this figure, it seems that our paper is a system paper.
%     % overview of the pipeline in order to introduce the relationship
%     % between the subsections.
%     % \fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
%     \includegraphics[width=1\linewidth]{figures/pipeline}
%     \caption{pipeline of the algorithm [todo] add more info in the caption.}
%     \label{fig:pipeline}
% \end{figure*}

% [coarse] --> [fine]
% [coarse]: global / inter-volume surface interaction
% [fine]: local / intra-volume surface prediction
% Limited by the hardware memory size, the proposed algorithm is in a sliding 3D cube manner.  
% A bounded 3D space is covered by a set of overlapping voxel cubes $\bm{C}$,
%     each \textit{center voxel} of which is represented as $\dot{x}$.
% So that the multiview stereopsis can be observed as 
%     the reconstruction of surface segments $\bm{C}_{\bm{I}}^s = \{c_1^s,c_2^s,...,c_i^s\}$ 
%     from all the voxel cubes $\bm{C}_{\bm{I}} = \{c_1,c_2,...,c_i\}$,
%     where $\bm{I}=\{\dot{x}\}$.
% The voxel in $c_i^s$ has boolean attribute, i.e. $x^s \in \{0,1\}$.
% \par
% 
% % CNN + simple assemblage
% A convolutional neural network (CNN), called surfaceNet, is applied 
%     to recover fine geometric structure within each voxel cube 
%     $c \in \bm{C}$ according to its appearance on different views $\bm{v} = \{v_1,v_2,...v_j\}$,
%     the view patches $\bm{P_c} = \{P(c,v)|v \in \bm{v}\}$.
% \par
% 
% % edge detection: 1D from 2D ==> MVS: 2D from 3D
% The design of the surfaceNet is inspired by the works on 
%     object boundary detection \cite{xie2015holistically}, which predicts 1D boundary from 2D image input.
% Analogically, the MVS problem could be considered as a 2D surface reconstruction from 3D voxel space.
% \par  
% 
% % section outlier 
% In the following sections, we firstly consider how to predict accurate 3D surface segment
%     in each local voxel cube using neural network.
% Then schemes to speed up and to refine the results will be discussed.
% \par

We propose an end-to-end learning framework that takes a set of images and their corresponding camera parameters as input and infers the 3D model.
To this end, we voxelize the solution space and propose a convolutional neural network (CNN) that predicts for each voxel $x$ a binary attribute $s_x \in \{0,1\}$ depending on whether the voxel is on the surface or not. We call the network, which reconstructs a 2D surface from a 3D voxel space, \textit{SurfaceNet}. It can be considered as an analogy to object boundary detection \cite{xie2015holistically}, which predicts a 1D boundary from 2D image input. 

We introduce SurfaceNet in Section~\ref{intraVolume} first for the case of two views and generalize the concept to multiple views in Section~\ref{multiViewFusion}. In Section~\ref{implementation} we discuss additional implementation details like the early rejection of empty volumes that speed up the computation.   






==> sections/_x_-results.tex <==
%= = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = =
\subsection{Dataset}\label{dataset}

%- - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - 
%\subsection{training process} \label{train}
% about the DTU dataset
The DTU multi-view stereo dataset \cite{aanaes2016large} is a large scale MVS benchmark.
It features a variety of objects and materials, 
    and contains 80 different scenes seen from 49 or 64 camera positions 
    under seven different lighting conditions. The provided reference models are acquired by accurate structured light scans.
    The large selection of shapes and materials is well-suited to train and test our method under realistic conditions and the scenes are complex enough even for the state-of-the-art methods, 
    such as \textit{furu}~\cite{furu2010accurate}, \textit{camp}~\cite{campbell2008using}, \textit{tola}~\cite{tola2012efficient} and  \textit{Gipuma}~\cite{galliani2015massively}.  
% train/val/test set
For evaluation, we use three subsets of the objects from the DTU dataset
    for training, validation and evaluation.
%The selected scenes in each subset are listed in the supplementary material.
\footnote{Training: 
        2, 6, 7, 8, 14, 16, 18, 19, 20, 22, 30, 31, 36, 39, 41, 42, 44, 45, 46, 47, 50, 51, 52, 53, 
        55, 57, 58, 60, 61, 63, 64, 65, 68, 69, 70, 71, 72, 74, 76, 83, 84, 85, 87, 88, 89, 90, 91, 
        92, 93, 94, 95, 96, 97, 98, 99, 100, 101, 102, 103, 104, 105, 107, 108, 109, 111, 112, 
        113, 115, 116, 119, 120, 121, 122, 123, 124, 125, 126, 127, 128. Validation: 3, 5, 17, 21, 28, 35, 37, 38, 40, 43, 56, 59, 66, 67, 82, 86, 106, 117. Evaluation: 1, 4, 9, 10, 11, 12, 13, 15, 23, 24, 29, 32, 33, 34, 48, 49, 62, 75, 77, 110, 114, 118}
    
    
The evaluation is based on \textit{accuracy} and \textit{completeness}. 
Accuracy is measured as the distance from the inferred model to the reference model, 
    and the completeness is calculated the other way around. Although both are actually error measures and a lower value is better, we use the terms \textit{accuracy} and \textit{completeness} as in \cite{aanaes2016large}.
%The smaller the measurements are, the better the evaluated result is. 
%\textbf{Ji: Since the DTU dataset also mentions that their scanned model cannot be called ground truth model, 
%    they call it reference model. Few reference paper use the term 'ground truth'.}
%\textit{do we need to mention the complexity? around 10 hours / model when $N_v=5$. Half of the time is wasted on the low efficiency code.}
%\par
% voxel cube size s = 32
Since the reference models of the DTU dataset are down-sampled to a resolution of $0.2mm$ for evaluation, 
we set the voxel resolution to $0.4mm$. % which is close to the down-sampled resolution of the reference models of the DTU dataset \cite{aanaes2016large}. %A finer resolution would therefore not improve the results of the quantitative evaluation. 
In order to train SurfaceNet with a reasonable batch size, we use cubes with $32^3$ voxels.      

%The voxel resolution is decided by how fine the 3D structure want to be reconstructed.
%For the DTU dataset \cite{aanaes2016large}, it is set to $r=0.4mm$.

%Balancing between the limited GPU memory that limits the largest voxel cube shape and 
%    the requirement for the geometric structure representation power of voxel cube,
%    we set the cube shape parameter $s=32$.
% voxel resolution r = 0.4mm

%\par

% why choose DTU
% The large selection of shapes and materials is well-suited to train and test our method under realistic conditions.
% Importantly, the scenes are complex enough even for the state-of-the-art methods, 
%     such as \textit{furu}\cite{furu2010accurate}, \textit{camp}\cite{campbell2008using}, and \textit{tola}\cite{tola2012efficient}.
% % train/val/test set
% In our method, we use three subsets of objects from the extensive DTU dataset
%     for training, validation and evaluation.
% The selected scenes in each subset are mentioned in the Appendix.
% \par
%
%\textbf{Train surfaceNet:}
%The 3D surfaceNet is trained from scratch.
%% input samples and reference
%In the groud truth 3D surface model, using binary to indicate the occupancy information of each voxel, 
    %a volume of voxel $c$ with boolean occupancy attributes is defined as $c^{gt}$ and is treated as the supervision of the network.
%For the input sample, we use $N_v^{train}=6$ pairs of CVCs from randomly selected view pairs.
%% how to choose N_v during training
%Since at the very beginning the view pair selection module is not available and
    %some selected views could be severely blocked, the $N_v^{train}$ cannot be too small.
%Meanwhile, large set of colored voxels take huge amount of GPU memory with the fixed batch size.
%\par
%
%% seperately train the 3D CNN & the relative importance
%The surfaceNet and the relative importance $w(c,v_i,v_j)$ are not trained at one shot,
    %since the relative importance only makes sense and can be trained 
    %before the surfaceNet outputs $c^p$ meaningful surface prediction.
%% if train together, the 2 modules will misleading each other --> low training efficiency
%If the noisy surfaceNet outputs $c^p$ misleading the relative importance, 
    %which acts as the weight during the weighted average operation,
    %the affected relative importance module inversely infuences the training efficiency of the 3D CNN module.
%\par
%
%% train the 3D CNN module
%Firstly, we train the surfaceNet module from scratch by modifying the weighted average fusion 
    %into a mean average operation, so that the relative importance module can be temporally ignored.
%% preprocessing and data augmentation
%For all the colored cubes, we first subtracted the VGG \cite{simonyan2014very} mean color vector
    %commonly used in the image applications, 
    %and then perform extensive data augmentation in order to combat overfitting of the model and improve the generalization.
%\par 
%% train the relative importance module
%Secondly, the relative importance module, i.e. $r(\cdot)$, is trained by keeping the above learned surfaceNet model.
%\par
%
%\textbf{Train $d(c,v_i,v_j)$:}
%% prepare training set
%Recall that a triplet network followed by a logistic regressor $l(\cdot)$ is trained.
%One thing need to mention is how to prepare the training data.
%Some 3D on/off-surface points can be randomly sampled 
    %from the ground truth model surface to generate positive / negtive labels.
%A voxel cube $c$ is projected onto any pair of views 
    %$(v_i,v_j)$ to crop a pair of image patchs $P(c,v_i),P(c,v_j)$, which are considered as a input sample.
%% sparse initialization
%When $d(c,v_i,v_j)$ is trained, the sparse initialization can be generated using \ref{eq:sparseInit} 
    %by setting $N_{min}=6$ for the 49 views in the DTU dataset.
%\par

% lasagne
%We used the public available \textit{Lasagne} Library \cite{lasagne} to implement the network structure.
%The training process takes roughly 5 days using a Nvidia TITAN X GPU.
%\par

%\input{sections/fig/tau.tex}
\input{sections/fig/tau_gamma.tex}

%- - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - 
\subsection{Impact of Parameters}
% \tau, \gamma, \beta, N_v

We first evaluate the impact of the parameters for binarization. In order to provide a quantitative and qualitative analysis, we use model 9 of the dataset, which was randomly chosen from the test set. By default, we use cubes with $32^3$ voxels.   
%In this subsection, we discuss the setting for each parameter. 
%The effect of each parameter is illustructed using the reconstruction results on a randomly choosen test model (model 9).
%\par
 
As discussed in Section \ref{multiViewFusion:inf}, the binarization depends on the threshold $\tau$ and the parameter $\gamma$ for thinning. If $\gamma=0\%$ thinning is not performed. Fig.~\ref{fig:tau_gamma} shows the impact of $\tau$ and $\gamma$. 
%for the three cases for each parameter: $\tau=0.5,0.7,0.9$ and $\gamma=0\%,50\%,100\%$. 
For each parameter setting, the front view and the intersection with a horizontal plane (red) is shown from top view. The top view shows the thickness and consistency of the reconstruction.
%
%of a horizontally selected piece of points 
% in order to give a sense about the photoconsistency by checking the thickness of the plane section view.
% 
We observe that $\tau$ is a trade-off between accuracy and completeness. While a large value $\tau=0.9$ discards large parts of the surface, $\tau=0.5$ results in a noisy and inaccurate reconstruction. The thinning, \ie $\gamma=100\%$, improves the accuracy for any threshold $\tau$ and slightly impacts the completeness.      
  

% As SurfaceNet directly outputs voxel probability of being on surface or not,
%     a large model is reconstructed in sliding cube manner.
% The most straightforward way to get the model surface is simply applying an universal threshold $\tau$ 
%     to all the voxels coved by the sliding cubes for binarilization, 
%     as shown in the case of $\gamma=0\%$ in Fig.~\ref{fig:tau}.
% Obvisouly, as $\gamma$ getting larger the less confident voxels are gradually filtered out.
% In the large $\tau=0.9$ case, even the potientially good surface is also be damaged.
% And the ray pooling operation, i.e. $\gamma > 0\%$, does not affect the trend of accuracy and completeness.
% \par


% \input{sections/fig/gamma.tex}

%%% In Fig.~\ref{fig:tau_gamma} we show the impact of $\gamma$. In contrast to the trade-off parameter $\tau$, the thinning improves the results qualitatively and quantitatively. The surface gets not only thinner, but the accuracy is also substantially improved while the impact on the completeness is minor. For $\tau=0.5$ the accuracy is drastically improved, but even for $\tau=0.7$ the improvement in accuracy is substantial. For instance, the red artifacts in front of the gray facade for $\gamma=0\%$ gets removed for $\gamma\geq80\%$. Since the thinning removes points, the completeness slightly decreases. This can be seen at the chimney where the hole for $\gamma=100\%$ is slightly larger than for $\gamma=80\%$.             


% Since the binarilization leads to thick 3D surface, the importance of the ray pooling operation is reflected
%     from Fig.~\ref{fig:gamma}.
% In the both cases $\tau=0.5;0.7$ the ray pooling is constantly boost the accuracy of the reconstruction model
%     with tiny loss on completeness metric,
%     as only the voxels with higher probability along the view rays direction are left.
% Notice from the figures that the ray pooling has two kinds of effects:
%     1. as the thick surface wraps the real surface 
%     and blocks the sight to observe the true surface,
%     the thinning of ray pooling can ease the blocky artifact to some extend;
%     2. for some homogeneous region SurfaceNet may predict obviously erroneous surface that 
%     is nearly perpendicular to the view's image plane.
% \par

\input{sections/fig/beta.tex}
\input{sections/fig/iter.tex}

While the threshold $\tau=0.7$ seems to provide a good trade-off between accuracy and completeness, we also evaluate the approach described in Section \ref{adaptivethres} where the constant threshold $\tau$ is replaced by an adaptive threshold $\tau_C$ that is estimated for each cube by minimizing~(\ref{eq:E}) iteratively. The energy, however, also provides a trade-off parameter $\beta$~(\ref{eq:psi}). If $\beta$ is large, we prefer completeness and when $\beta$ is small we prefer accuracy.      
This is reflected in Fig.~\ref{fig:beta} where we show the impact of $\beta$. 
%Note that in contrast to Figures~\ref{fig:tau_gamma} and~\ref{fig:tau_gamma}, the red artifacts in front of the gray facade are removed. 
Fig.~\ref{fig:iter} shows how the reconstruction improves for $\beta=6$ with the number of iterations from the initialization with $\tau_C=0.5$. The method quickly converges after a few iterations. By default, we use $\beta=6$ and 8 iterations for the adaptive binarization approach.         



% 
% There are several drawbacks of the universal thresholding scheme:
%     1. need user defined or model specific threshold $\tau$;
%     2. do not consider the neighboring surface for reconstruction, so that it leads to eather lots of floating noise or many holes.
% The adaptive threshold is proposed to dynamicly balance between the noise and holes and 
%     to find individual threshold in each cube by considering the information of the connecting surface.
% In (\ref{eq:psi}) the parameter $\beta$ is a tradeoff between the mismatch penalization and the connectivity encourage for the overlapping surface.
% Obviously, the larger $\beta$ is, the more complete the model be.
% 
% That is also reflected in Fig.~\ref{fig:beta}, except the value $\beta=0$, other candidate settings have the similiar performance
%     regarding to the tradeoff between the holes and the noise in the model.
% As a result, $\beta$ is assigned to $6$. 
% Finally, the adaptive threshold procedure is done by iteratively solving (\ref{eq:psi}) using numerical gradient descent.
% The intermediat results are listed in Fig.~\ref{fig:iter}, showing that the algorithm converge within few iterations.
% \par


\begin{table}[htbp]
\centering
\small
%\hspace{-0.5cm}
\begin{tabular}{ccccc}
methods (mm) & \begin{tabular}{@{}c@{}}mean \\ acc\end{tabular}
        & \begin{tabular}{@{}c@{}}med \\ acc\end{tabular}
        & \begin{tabular}{@{}c@{}}mean \\ compl\end{tabular}
        & \begin{tabular}{@{}c@{}}med \\ compl\end{tabular} \\
    \hline
    $\tau=0.7$ $\gamma=0\%$ &             0.574	&0.284    &\textbf{0.627}	&\textbf{0.202} \\
    \hline
    $\tau=0.7$ $\gamma=80\%$ &          0.448	&\textbf{0.234}	&0.706	&0.242 \\
    \hline
    adaptive threshold \\ $\beta=6$ $\gamma=80\%$ &   \textbf{0.434}	&0.249	&0.792	&0.229 \\
    \hline
    adaptive threshold \\ $\beta=6$ $\gamma=80\%$ \\ w/o weighted average &  0.448 &   0.251 &       0.798 & 0.228 \\
    \hline
\end{tabular}
%\hspace{0.3cm}
% put caption below the \end{tabular} to put the caption at the bottom
\captionof{table}{
A quantitative comparison of two well performing parameter settings for $\tau$ and $\gamma$ with the adaptive binarization procedure. The last row reports the result when the view pairs are not weighted.
    The evaluation is performed for the model~9.
} \label{tab:adapthresh}
\end{table}

We compare the adaptive binarization with the constant thresholding in Table~\ref{tab:adapthresh} where we report mean and median accuracy and completeness for model 9. The configuration $\tau=0.7$ and $\gamma=80\%$ provides a good trade-off between accuracy and completeness. Using adaptive thresholding with $\beta=6$ as described in Section~\ref{adaptivethres} achieves a better mean accuracy but the mean completeness is slightly worse. We also report in the last row the result when the probabilities $p_x$ are not weighted in (\ref{eq:fusion}), \ie, $w_C^{(v_i,v_j)}=1$. This slightly deteriorates the accuracy.           




% To illustrate the improvement of the adaptive threshold, 
%     Tab.\ref{tab:adapthresh} compares with two representitive configurations of $\tau$ and $\gamma$ with good performance.
% As shown in the table, the adaptive threshold improves the result from both the accuracy and the completeness aspects.
% Be consistent with the previous comparisons, this table is also evaluated on model 9, which is randomly chosen in the test set.
% In the table, we also compare the same adaptive threshold algorithm with different fusion schemes.
% The weighted fusion is as mentioned in (\ref{eq:fusion}), 
%     compared with a mean average by simply averaging surface predictions from multiple view pairs.
% From the table we can conclude that the weighted average is crucial for the accuracy and 
%     the infered weights in (\ref{eq:relativeImportance}) works as expected.
% At the same time, in order to further test our view selection module, 
%     all the inference listed in the paper considers all the possible view pairs as candidates without pre-selection.
% \par




\input{sections/fig/Nv.tex}

We finally evaluate the impact of fusing the probabilities $p_x$ of the best $N_v$ view pairs in (\ref{eq:fusion}). By default, we used $N_v=5$ so far. The impact of $N_v$ is shown in Fig.~\ref{fig:Nv}. While taking only the best view pair results in a very noisy inaccurate reconstruction, the accuracy is substantially improved for three view pairs. After five view pairs the accuracy slightly improves at the cost of a slight deterioration of the completeness. We therefore keep $N_v=5$.          

% In Section~\ref{multiViewFusion}, we define the number of view pairs used for surface reconstruction as $N_v$.
% Intuitively, the reconstruction time is nearly proportial to $N_v$.
% Aditionally, it is also a tradeoff term regarding to accuracy and completeness, as infered from Fig.~\ref{fig:Nv}.
% When we only consider one view pair, the accuracy is not good inspite of high completeness.
% As $N_v$ gets larger, the performance do not have big difference considering both accuracy and completeness.
% \par

\input{sections/fig/more.tex}


%- - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - 
\subsection{Comparison with others methods}

\begin{table}[t]
% \hspace{0.2cm}
%\small
\footnotesize
\centering
%\hspace{-0.3cm}
\begin{tabular}{ccccc}
    methods (mm) & \begin{tabular}{@{}c@{}}mean \\ acc\end{tabular}
        & \begin{tabular}{@{}c@{}}med \\ acc\end{tabular}
        & \begin{tabular}{@{}c@{}}mean \\ compl\end{tabular}
        & \begin{tabular}{@{}c@{}}med \\ compl\end{tabular} \\
    \hline
    \textit{camp} [1]    &         0.834 &   0.335 &   \textbf{0.987} & \textbf{0.108} \\
    \textit{furu} [2]    &          0.504 &   0.215 &   1.288 & 0.246 \\
    \textit{tola} [3]    &             0.318 &   0.190 &   1.533 & 0.268 \\
    \textit{Gipuma} [4]    &    \textbf{0.268} &   \textbf{0.184} &   1.402 & 0.165 \\
    \hline
    \textit{SurfaceNet}    &    0.454 & 0.191 & 1.354 & 0.164 \\
    \hline
\end{tabular}
\captionof{table}{
    Comparison with other methods. The results are reported for the test set consisting of 22 models.
} \label{tab:compare_methods}
\end{table}

We finally evaluate our approach on the test set consisting of 22 models and compare it with the methods \textit{camp} \cite{campbell2008using}, \textit{furu} \cite{furu2010accurate}, \textit{tola} \cite{tola2012efficient}, and \textit{Gipuma} \cite{galliani2015massively}. While we previously used cubes with $32^3$ voxels, we also include the results for cubes with $64^3$ voxels in Table~\ref{tab:compare_methods}. Using larger cubes, \ie $s=64$, improves accuracy and completeness using a constant threshold $\tau=0.7$ with $\gamma=0\%$ or $\gamma=80\%$. When adaptive thresholding is used, the accuracy is also improved but the completeness deteriorates.      

If we compare our approach using the setting $s=64$, $\tau=0.7$, and $\gamma=80\%$ with the other methods, we observe that our approach achieves a better accuracy than \textit{camp} \cite{campbell2008using} and \textit{furu} \cite{furu2010accurate} and a better completeness than \textit{tola} \cite{tola2012efficient} and \textit{Gipuma} \cite{galliani2015massively}. Overall, the reconstruction quality is comparable to the other methods. A qualitative comparison is shown in Fig.~\ref{fig:methods}.
%However, given that the proposed approach is the first end-to-end learning framework for MVS, we further improvement either by         




% As shown in Table~\ref{tab:compare_methods}, our approach with the non-adaptive binarization achieves a better completeness than the other methods for any value of $\gamma$ and outperforms \textit{camp} \cite{campbell2008using} and \textit{furu} \cite{furu2010accurate} in terms of accuracy and completeness. The results of the adaptive binarization are comparable to \textit{tola} \cite{tola2012efficient} and \textit{Gipuma} \cite{galliani2015massively}. While our method is slightly worse in terms of accuracy, it is slightly better in terms of completeness.  

 



%- - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - 
\subsection{Runtime}

The training process takes about 5 days using an Nvidia Titan X GPU.
The inference is linear in the number of cubes and view pairs. 
For one view pair and a cube with $32^3$ voxels, inference takes 50ms. If the cube size is increased to $64^3$ voxels, the runtime increases to 400ms. However, the larger the cubes are the less cubes need to be processed. In case of $s=32$, model 9 is divided into 375k cubes, but most of them are rejected as described in Section~\ref{implementation} and only 95k cubes are processed. In case of $s=64$, model 9 is divided into 48k cubes and only 12k cubes are processed. 
%Note that larger cubes also improve the results (Table XX).


%- - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - 
\subsection{Generalization}

\begin{table}[htbp]
\centering
%\small
\footnotesize
\begin{tabular}{ccccc}
methods (mm) & \begin{tabular}{@{}c@{}}mean \\ acc\end{tabular}
        & \begin{tabular}{@{}c@{}}med \\ acc\end{tabular}
        & \begin{tabular}{@{}c@{}}mean \\ compl\end{tabular}
        & \begin{tabular}{@{}c@{}}med \\ compl\end{tabular} \\
    \hline
    49 views \\ \footnotesize$s=32$,  adapt $\beta=6$,  $\gamma=80\%$ &    0.197 &   0.149 &   1.762 & 0.237 \\
            \footnotesize$s=64$, $\tau=0.7$, $\gamma=80\%$    &    0.256 & 0.122 & \textbf{0.756} & \textbf{0.193} \\
    \hline
    15 views \\ \footnotesize$s=32$,  adapt $\beta=6$,  $\gamma=80\%$ &  \textbf{0.191}   &   0.135 &   2.517 & 0.387 \\
            \footnotesize$s=64$, $\tau=0.7$, $\gamma=80\%$    &    0.339 & \textbf{0.117} & 0.971 & 0.229 \\
    \hline
\end{tabular}
\captionof{table}{ 
Impact of the camera setting. The first two rows show the results for the 49 camera views, which are the same as in the training set. The last two rows show the results for 15 different camera views that are not part of the training set.   
The evaluation is performed for the three models 110, 114, and 118.
} \label{tab:15views}
\end{table}

In order to demonstrate the generalization abilities of the model, we apply it to a camera setting that is not part of the training set and an object from another dataset.  

The DTU dataset \cite{aanaes2016large} provides for some models additional 15 views which have a larger distance to the object. For training, we only use the 49 views, which are available for all objects, but for testing we compare the results if the approach is applied to the same 49 views used for training or to the 15 views that have not been used for training. In our test set, the additional 15 views are available for the models 110, 114, and 118. The results in Table \ref{tab:15views} show that the method performs very well even if the camera setting for training and testing differs. While the accuracy remains relatively stable, an increase of the completeness error is expected due to the reduced number of camera views.    

\input{sections/fig/middlebury.tex}

We also applied our model to an object of the Middlebury MVS dataset \cite{seitz2006comparison}. We use
6 input images from the view ring of the model dinoSparseRing for reconstruction. The reconstruction is shown in Fig.~ \ref{fig:middlebury}.


% % 15 views for DTU dataset
% In the training stage, we used the 49 views which are available for all models in the DTU dataset. 
% In order to show the generalization of the trained model, two sets of different camera settings are used for reconstruction.
% \par
% 
% The DTU dataset \cite{aanaes2016large} also provides for some models additional 15 views which have a larger distance to the object. 
% We use our trained model on the 49 views and apply it only to the 15 views, i.e., the camera views of the training and test set differ. 
% The test models 110/114/118 has the extra 15 views available
% The result for these models are listed in \ref{tab:15views}.  
% Because of the sparser views, the selected view pairs have large baseline to improve the accuracy.
% At the same time, few views observe less of the model surface, and obviously has negative impact on the completeness.
% Therefore, the tiny change between the two set of views in \ref{tab:15views} 
%         can prove that our model trained on a specific set of views can can be generalized for a different set of camera settings.
% \par
% 
% \input{sections/fig/middlebury.tex}
% 
% As illustrated in \ref{fig:middlebury}, the trained model can be also generalized to other dataset, such as the Middlebury MVS dataset \cite{seitz2006comparison}.
% 6 input images are selected from the view ring of the model dinoSparseRing to be used for reconstruction.
% One of the input images is like the top right image.
% The reconstruction result and a plane section view of the selected piece of points are seperately listed.
% The good plane section view can visualize the photoconsistency the model has learned.
% This can also prove the generalization property of our method and the trained model.
% % 6 views for middlebury dinoSparseRing model, with settings: views={7..12}, cubeSize=64, \beta=70, 
% \par



% models for evaluation: 33, 32, 29, 15, 13, 12, 11, 10, 9, 4, 1,

% \textbf{todo:} mention the most recent method \cite{7780960}, without code.
% 
% To further proof each postprocessing modules, we list 4 setting of our methods:
%     1. universal thresholding $\tau=0.7$ without ray pooling, i.e. $\gamma=0\%$;
%     2. $\tau=0.7$ with ray pooling by setting the user defined parameter $\gamma=80\%$;
%     3. change the above fix threshold to adaptive threshold.
%     4. simply reserve the voxels voted by all the views, i.e. $\gamma=100\%$.
% 
% It turns out that case 1. has the worse accuracy and best completeness.
% As $\gamma$ increases, the accuracy is improved with tiny loss on the completeness.
% Among all the settings, the adaptive threshold can further boost the accuracy.
% Compared with other methods:
%     ours is better than \textit{furu}, \textit{camp}, and \textit{tola}, and is competetive with \textit{Gipuma}.

%\input{sections/fig/more.tex}



==> sections/_x_-surfaceNet.tex <==
\section{SurfaceNet}\label{intraVolume}

% % use CNN for intra-volume prediction
% Given a sequence of posed images the multi-view stereo problem is to reconstruct a 3D model.
% In this section, we only consider how to recover accurate geometric details
%     in each local voxel volume from ONE visible non-occluded view pair.
% As has been previously mentioned, the proposed method trains
%     a CNN to densely predict the occupancy probability at voxel position.
% Unlike the depth map fusion approaches,
%     such data driven method can easily learn a high level representation of the
%     3D structure information without carefully designed procedures.
% \par
%
% % design network for MVS is not trivial. input image with output of 3D model
% Despite the representative power of deep networks,
%     naively training a deep network to predict 3D surface structure
%     by supplying the set of images as inputs directly is unlikely to work well,
%     for several key reasons.
% \par
%
% % [reason1] hard to learn perspective projection (2D <--> 3D in each view)
% First, the pose parameters of the views would need to be supplied
%     as inputs to the network in order to produce the desired 3D surface.
% The relationship between the pose parameters,
%     the input pixels and the output surface voxel is complex and non-linear.
% The network would need to learn how to interpret rotation angles and perform image reprojection.
% Forcing the network to learn projection is inefficient.
% But it is a straightforward operation that we can represent outside of the network.
% \par
%
% % [reason2] hard to embed epipolar constraint (relationship between views)
% Second, in order to reconstruct the 3D surface from the images from non-fixed poses,
%     the network would need to compare and combine potentially distant pixels in
%     different view images, necessitating very dense and long-range connections.
% Such a network would have many parameters and would be slow to train,
%     prone to overfitting, and slow to run inference on.
% A network structure could be designed to use the epipolar constraint internally
%     in order to limit connections to those on corresponding epipolar lines.
% However, the epipolar lines would be pose-dependent,
%     making this very difficult and likely computationally inefficient in practice.
% \par
Given two images $I_i$ and $I_j$ for two views $v_i$ and $v_j$ of a scene with known camera parameters and a voxelization of the scene denoted by a 3D tensor $C$, %and all voxels $x\in C$ that belong to C, 
our goal is to reconstruct the 2D surface in $C$ by estimating for each voxel $x\in C$ if it is on the surface or not, \ie $s_x \in \{0,1\}$.

To this end, we propose an end-to-end learning framework, which automatically learns both photo-consistency and geometric relations of the surface structure. Intuitively, for accurate reconstruction, the network requires the images $I_i$ and $I_j$ as well as the camera parameters. However, direct usage of $I_i$, $I_j$ and their corresponding camera parameters as input would unnecessarily increase the complexity of the network since such network needs to
learn the relation between the camera parameters and the projection of a voxel onto the image plane in addition to the reconstruction. Instead, we propose a 3D voxel representation that encodes the camera parameters implicitly such that our network can be fully convolutional.




%- - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - -
% \subsection{Colored voxel cube}
% % why 2D --> 3D
% To explicitly provide the perspective projection information and the epipolar constraint
%     to the CNN, we introduce \textit{colored voxel cube} (CVC) $c^*(v_j)$ with respective to view $v_j$.
% \par

\begin{figure}[h] % t/b/h: put the figure at the top / bottom / here
\centering
    \includegraphics[width=0.8\linewidth]{figures/coloredCube} % scale=1 / width=0.8\linewidth\textwidth
    \caption{Illustration of two Colored Voxel Cubes (CVC).}
    \label{fig:coloredCube}
\end{figure}

We denote our representation as \textit{colored voxel cube} (CVC), which is computed for each view and illustrated in Fig.~\ref{fig:coloredCube}. For a given view $v$, we convert the image $I_v$ into a 3D colored cube $I^C_v$ by projecting each voxel $x \in C$ onto the image $I_v$ and storing the RGB values $i_x$ for each voxel respectively. For the color values, we subtract the mean color~\cite{simonyan2014very}.
Since this representation is computed for all voxels $x \in C$, the voxels that are on the same projection ray have the same color $i_x$. In other words, the camera parameters are encoded with CVC. As a result, we obtain for each view a projection-specific stripe pattern as illustrated in Fig.~\ref{fig:coloredCube}.






% As shown in \figref{coloredCube}, a voxel $x$ in $c$ is corresponding to a pixel
%     $p(v_j,x)$ on view $v_j$ by perspective projection.
% The colored voxel cube $c^*(v_j)$ with respective to view $v_j$ is defined by
%     colorizing each voxel $x$ in $c$ using the color vector (RGB or gray) of $p(v_j,x)$.
% \par
%
% Using CVC as inputs to the neural network removes the need
%     to supply the pose parameters since they are now implicitly embedded during
%     the CVCs construction.
% Additionally, the epipolar constraint is trivially enforced within a pair of CVCs
%     that could have dissimilar appearance from different view patches $p \in \bm{P_c}$,
%     based on which $c^*(v_i)$ is defined.
% That means that it avoids epipolar rectification and allows one to aggregate evidence over multiple iamges.
% \par
%
% % voxel cube size s = 32
% Balancing between the limited GPU memory that limits the largest voxel cube shape and
%     the requirement for the geometric structure representation power of voxel cube,
%     we set the cube spatial dimentions as $s\times s\times s$, $s=32$.
% % voxel resolution r = 0.4mm
% The voxel resolution is decided by how fine the 3D structure want to be reconstructed.
% In the DTU dataset \cite{aanaes2016large}, it is set to $r=0.4mm$.
% \par


%- - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - -
\subsection{SurfaceNet Architecture}

% % CVC and c^{*}
% As illustrated in \figref{surfaceNet}, a voxel cube $c \in \bm{C}$ could have
%     dissimilar appearance from different view $v_i \in \bm{v}$,
%     based on which a colored voxel cube of $c$
%     with respect to $v_i$ is defined as $c^{*}(v_i)$.
% Since $c^{*}(v_i)$ is the intersection between the voxel cube $c$ and the CVC of $v_i$,
%     each voxel position of $c^{*}(v_i)$ has RGB three color channels.
% \par
%
% % Traditionally: individual voxel recovery
% Traditionally, depth map fusion methods produce 2D dpth maps as intermediate results
%     and don't consider 3D structure information directly.
% % ours: recovers set of voxels
% In contrast, the proposed network takes as input a pair of colored voxel cubes
%     $c^{*}(v_1), c^{*}(v_2)$ induced from view patches $P(c,v_1)$ and $P(c,v_2)$
%     learns the 3D structure information, and directly outputs a 3D surface segment
%     $c^s$ without lengthy steps.
% \par
%
% % $c^p$ and $c^s$
% Note that each voxel in $c^s$ has boolean attribute indicating
%     whether the voxel is occuppied as a partical of the surface segment.
% Similarly we define the \textbf{probability cube} as $c^p$, voxel value of which stands for
%     the occupancy probability of that voxel $x^p \in [0,1]$.
% $c^s$ can be simply got by binarilization using threshold $\overline{t}_c \in [0,1]$.



\begin{figure}[htbp] % t/b/h: put the figure at the top / bottom / here
\centering
\includegraphics[width=\linewidth]{figures/surfaceNet} % scale=1 / width=0.8\linewidth\textwidth
\caption{SurfaceNet takes two CVCs from different viewpoints as input.
    Each of the RGB-CVC is a tensor of size $3 \times s \times s \times s$.
    In the forward path, there are four groups of convolutional layers. The $l_{4.\cdot}$ layers are 2-dilated convolution layers.
    The side layers $s_{i}$ extract multi-scale information, which are aggregated into the output layer $y$
        that predicts the on-surface probability for each voxel position. The output has the size $1 \times s \times s \times s$.}
\label{fig:surfaceNet}
\end{figure}
% CVC and c^{*}
The architecture of the proposed SurfaceNet is shown in Fig.~\ref{fig:surfaceNet}. It takes two colored voxel cubes from two different viewpoints as input and predicts for each voxel $x \in C$ the confidence $p_x \in (0,1)$, which indicates if a voxel is on the surface. While the conversion of the confidences into a surface is discussed in Section~\ref{inference}, we first describe the network architecture.

The detailed network configuration is summarized in Table~\ref{table:3DCNN-tab}. The network input is a pair of colored voxel cubes, where each voxel stores three RGB color values. For cubes with $s^3$ voxels, the input is a tensor of size $6\times s\times s\times s$. The basic building blocks of our model are 3D convolutional layers $l(\cdot)$, 3D pooling layers $p(\cdot)$ and 3D up-convolutional layers $s(\cdot)$,
where $l_{n.k}$ represents the $k$th layer in the $n$th group of convolutional layers. Additionally, a rectified linear unit (ReLU) is appended to each convolutional layer $l_i$ and the sigmoid function is applied to the layers $s_i$ and $y$. In order to decrease the training time and increase the robustness of training, batch normalization \cite{ioffe2015batch} is utilized in front of each layer.
The layers in $l_4$ are dilated convolutions \cite{yu2015multi} with dilation factor of 2.
They are designed to exponentially increase the receptive field without loss of feature map resolution.
The layer $l_{5.k}$ increases the performance by aggregating multi-scale contextual information from the side layers $s_i$
    to consider multi-scale geometric features.
Since the network is fully convolutional, the size of the CVC cubes can be adaptive. The output is always the same size as the CVC cubes.






% % surfaceNet overview
% As demonstrated in \figref{surfaceNet}, the voxel cube $c$ is firstly colorized based on
%     view patches $P(c,v_1)$ and $P(c,v_2)$.
% Then the surfaceNet takes as input a pair of colored voxel cubes,
%     producing probability cubes.
% \par
%
% The basic building blocks of our model are convolutional layer $l(\cdot)$,
%     pooling layer $p(\cdot)$ and up-convolutional layer $s(\cdot)$.
% Where $l_{n.k}$ represents the $k$th layer in the $n$th group of convolutional layers.
% For illustration, we use 2D squares to represent 3D cubes.
% For example the shape of $c^*(v_2)$ is $3\times s\times s\times s$.
% The determination of the cube size is a balance between the GPU memory and
%     the amount of surface context coveraged by the cube.
% The detailed network configuration is summarized in table \ref{table:3DCNN-tab}.
% As the network input is a pair of colored voxel cubes, each of which has RGB color channels,
%     the input shape is $6\times s\times s\times s$.
% By default all the mentioned layers are 3D operations,
%     such as 3D convolutional layer and 3D pooling layers.
% \par
%
% % dilated convolution
% Note that the layers $l_4$ is designed to increase the performance of
%     dense prediction architectures by aggregating multi-scale contextual information
%     using dilated convolution in \cite{yu2015multi},
%     which can exponentially increase the receptive field
%     without loss of feature map resolution.
% \par
%
% % nonlinear = ReLu
% Additionally, The ReLu nonlinear function is appended to each convolutional layer $l_i$,
%     and the Sigmoid function is applied to the final layers of $s_i$ and $l_{4.3}$.
% % batch normalization layer in front of conv layers.
% In order to chase fast and robust training, the batch normalization \cite{ioffe2015batch} is
%     utilized in front of each layers.
% \par


\begin{table}[htbp]
% \hspace{0.2cm}
% \centering
% \raggedleft
    \begin{tabular}{cccc} %{| p{5cm} | p{5cm} | p{5cm} |}
    \hline
    layer name & type & output size & kernel size \\
    \hline
    input                      & CVC         & $(6, s, s, s)$    & - \\
    $l_{1.1},l_{1.2},l_{1.3}$   & conv      & $(32, s, s, s)$    & $(3,3,3)$ \\
    $s_1$                       & upconv      & $(16, s, s, s)$    & $(1,1,1)$   \\
    $p_1$                       & pooling   & $(32, \frac{s}{2}, \frac{s}{2}, \frac{s}{2})$  & $(2,2,2)$  \\
    $l_{2.1},l_{2.2},l_{2.3}$   & conv      & $(80, \frac{s}{2}, \frac{s}{2}, \frac{s}{2})$    & $(3,3,3)$ \\
    $s_2$                       & upconv    & $(16, s, s, s)$    & $(1,1,1)$   \\
    $p_2$                       & pooling   & $(80, \frac{s}{4}, \frac{s}{4}, \frac{s}{4})$  & $(2,2,2)$  \\
    $l_{3.1},l_{3.2},l_{3.3}$   & conv      & $(160, \frac{s}{4}, \frac{s}{4}, \frac{s}{4})$    & $(3,3,3)$ \\
    $s_3$                       & upconv    & $(16, s, s, s)$    & $(1,1,1)$   \\
    $l_{4.1},l_{4.2},l_{4.3}$   & dilconv      & $(300, \frac{s}{4}, \frac{s}{4}, \frac{s}{4})$    & $(3,3,3)$ \\
    $s_4$                       & upconv    & $(16, s, s, s)$    & $(1,1,1)$   \\
    $l_{5.1},l_{5.2}$           & conv      & $(100, s, s, s)$    & $(3,3,3)$ \\
    $y$                       & conv    & $(1, s, s, s)$    & $(1,1,1)$   \\
    \hline
    \end{tabular}
\captionof{table}{Architecture of SurfaceNet. A rectified linear activation function is used after each convolutional layer except $y$,
       and a sigmoid activation function is used after the up-convolutional layers and the output layer to normalize the output.
} \label{table:3DCNN-tab}
\end{table}

\subsection{Training}
% define x \in X
As the SurfaceNet is a dense prediction network, \ie, the network predicts the surface confidence for each voxel, we compare the prediction per voxel $p_x$ with the ground-truth $\hat{s}_x$. For training, we use a subset of the scenes from the DTU dataset \cite{aanaes2016large} which provides images, camera parameters, and reference reconstructions obtained by a structured light system. A single training sample consists of a cube $\hat{S}^C$ cropped from a 3D model and two CVC cubes $I^C_{v_i}$ and $I^C_{v_j}$ from two randomly selected views $v_i$ and $v_j$.
Since most of the voxels do not contain the surface, \ie $\hat{s}_x=0$, we weight the surface voxels by
\begin{equation}
\alpha = \frac{1}{|\mathcal{C}|}\sum_{C \in \mathcal{C}}\frac{\sum_{x \in C}(1-\hat{s}_x)}{|C|}, 
\end{equation}
where $\mathcal{C}$ denotes the set of sampled training samples, and the non-surface voxels by $1-\alpha$. We use a class-balanced cross-entropy function as loss for training, \ie for a single training sample $C$ we have:
\begin{align} \label{eq:balancedEntropy}
    %L(C) = -\alpha \sum_{x^{y^+}}{\log x^p} - (1-\alpha) \sum_{x^{y^-}}{\log (1-x^p)}
    & L(I^C_{v_i},I^C_{v_j},\hat{S}^C) = \\
    &\nonumber\;- \sum_{x \in C} \left\{ \alpha \hat{s}_x \log p_x + (1-\alpha)(1-\hat{s}_x)\log (1-p_x) \right\}.
\end{align}
For updating the weights of the model, we use stochastic gradient descent with Nesterov momentum update.
\par

Due to the relatively small number of 3D models in the dataset, we perform data augmentation in order to reduce overfitting and improve the generalization. Each cube $C$ is randomly translated and rotated and the color is varied by changing illumination and introducing Gaussian noise.

%     we consider the objective function computing over each voxel $x^{(\cdot)} \in X_c^{(\cdot)}$ in a voxel cube $c$.
% $X_c^{(\cdot)}$ denotes the set of voxels in $c$ with attributes
%     like color $X_c^{*}$, probability $X_c^{p}$, and ground truth $X_c^{y}$.
% % biased +/- labels
% For a typical surface fragment, the distribution of surface/non-surface voxels,
%     $x^{y^+}\in X_c^{y^+}$ and $x^{y^-}\in X_c^{y^-}$, is heavily biased: the majority of the voxels have negative labels.
% We use a simple strategy to balance the loss between positive and negative classes.
% % class balanced cross entropy loss
% A class-balancing weight $p_{\Lambda}$ is introduced on a per-voxel term basis
%     to offset this imbalance between surface and non-surface voxels.
% Specifically, a class-balanced cross-entropy loss function for a specific sample in cube $c$ is defined as
% \begin{equation} \label{eq:balancedEntropy}
%     L_c = -\alpha \sum_{x^{y^+}}{\log x^p} - (1-\alpha) \sum_{x^{y^-}}{\log (1-x^p)}
% \end{equation}
%     where the voxel prediction $x^p \in X_c^p$ has range $[0,1]$,
%     the weight is estimated from the entire training samples $\alpha = \sum_{c}{(|X_c^{y^-}| / |X_c^{y}|)}$.
% \par

\subsection{Inference}\label{inference}
For inference, we process the scene not at once due to limitations of the GPU memory but divide the volume into cubes. For each cube, we first compute for both camera views the colored voxel cubes $I^C_{v_i}$ and $I^C_{v_j}$, which encode the camera parameters, and infer the surface probability $p_x$ for each voxel by the SurfaceNet. Since some of the cubes might not contain any surface voxels, we discuss in Section~\ref{implementation} how these empty cubes can be rejected in an early stage.

In order to convert the probabilities into a surface, we perform two operations. The first operation is a simple thresholding operation that converts all voxels with $p_x > \tau$ into surface voxels and all other voxels are set to zero. In Section \ref{adaptivethres}, we discuss how the threshold $\tau$ can be adaptively set when the 3D surface is recovered. The second operation is optional and it performs a thinning procedure of the surface since the surface might be several voxels thick after the binarization. To obtain a thin surface, we perform a pooling operation, which we call \textit{ray pooling}. For each view, we vote for a surface voxel $s_x=1$ if $x=\arg\underset{x' \in R}{\max}\; p_{x'}$, where $R$ denotes the voxels that are projected onto the same pixel. If both operations are used, a voxel $x$ is converted into a surface voxel if both views vote for it during ray pooling and $p_x > \tau$.




==> sections/acknowledgments.tex <==

%=========================================================================
\section*{Acknowledgments} % To get unnumbered chapters, parts, sections, subsections, etc
%\begin{acknowledgements}
%=========================================================================
%\section{acknowledgments} \label{acknowledgments}

The work has been supported in part by Natural Science Foundation of China (NSFC) under contract
No. 61331015, 6152211, 61571259 and 61531014, in part by the National key foundation
for exploring scientific instrument No.2013YQ140517, in part by Shenzhen Fundamental
Research fund (JCYJ20170307153051701) and in part by the DFG project GA 1927/2-2 as part of the DFG Research Unit FOR 1505 Mapping on Demand (MoD).

%\end{acknowledgements}


==> sections/fig/_x_-DTU_sparse.tex <==
\begin{figure*}[htbp]
    \centering
    \newcommand{\colw}{0.16}
    \newcommand{\figw}{1.0} % can bigger than 1
    \addtocounter{subfigure}{-4}
    \begin{minipage}[b]{0.03\textwidth}
        \begin{minipage}{\figw\textwidth}
            \vspace*{0.1cm}
            \rotatebox{90}{$\tau=0.5$}
        \end{minipage}
        \begin{minipage}{\figw\textwidth}
            \vspace*{0.1cm}
            \rotatebox{90}{$\tau=0.5$}
        \end{minipage}
        % \begin{subfigure}[t]{0.03\linewidth}
        \begin{minipage}{\figw\textwidth}
            \vspace*{0.1cm}
            \rotatebox{90}{$\tau=0.5$}
        \end{minipage}
   % \end{subfigure}%plot image
   % \begin{subfigure}[t]{0.03\linewidth}
        \begin{minipage}{\figw\textwidth}
            \vspace*{0.1cm}
            \rotatebox{90}{$\tau=0.5$}
        \end{minipage}
   % \end{subfigure}%plot image
    \end{minipage}%plot image
    \begin{minipage}[b]{\colw\textwidth}
        %\includegraphics[width=\figw\textwidth,trim={0cm 0cm 0cm 0cm},clip]{figures/results/model13/gt}
       
   % ~
        \begin{overpic}
         [width=1\textwidth,trim={0cm 0cm 0cm 0cm},clip]{figures/results/compare/DTU_sparse/model_1/surface+00_L00}\end{overpic}
        %\begin{overpic}[width=\figw\textwidth,trim={0cm 0cm 0cm 0cm},clip]{figures/results/model12/gt}\end{overpic}
        \begin{overpic}[width=\figw\textwidth,trim={0cm 0cm 0cm 0cm},clip]{figures/results/compare/DTU_sparse/model_1/rmvs00_L00}\end{overpic}
        \begin{overpic}[width=\figw\textwidth,trim={0cm 0cm 0cm 0cm},clip]{figures/results/compare/DTU_sparse/model_1/gipuma00_L00}\end{overpic}
        \captionof{subfigure}{dense}
        % \label{fig:sub1}
    \end{minipage}
    \begin{minipage}[b]{\colw\textwidth}
        %includegraphics[width=\figw\textwidth,trim={0cm 0cm 0cm 0cm},clip]{figures/results/model13/ours}
        \begin{overpic}[width=\figw\textwidth,trim={0cm 0cm 0cm 0cm},clip]{figures/results/compare/DTU_sparse/model_1/surface+00_L01}\end{overpic}
        %\begin{overpic}[width=\figw\textwidth,trim={0cm 0cm 0cm 0cm},clip]{figures/results/model12/ours}\end{overpic}
        \begin{overpic}[width=\figw\textwidth,trim={0cm 0cm 0cm 0cm},clip]{figures/results/compare/DTU_sparse/model_1/rmvs00_L01}\end{overpic}
        \begin{overpic}[width=\figw\textwidth,trim={0cm 0cm 0cm 0cm},clip]{figures/results/compare/DTU_sparse/model_1/gipuma00_L01}\end{overpic}
        \captionof{subfigure}{\textbf{Sparsity=3}}
    \end{minipage}
    \begin{minipage}[b]{\colw\textwidth}
        %includegraphics[width=\figw\textwidth,trim={0cm 0cm 0cm 0cm},clip]{figures/results/model13/furu}
        \begin{overpic}[width=\figw\textwidth,trim={0cm 0cm 0cm 0cm},clip]{figures/results/compare/DTU_sparse/model_1/surface+00_L02}\end{overpic}
        %\begin{overpic}[width=\figw\textwidth,trim={0cm 0cm 0cm 0cm},clip]{figures/results/model12/furu}\end{overpic}
        \begin{overpic}[width=\figw\textwidth,trim={0cm 0cm 0cm 0cm},clip]{figures/results/compare/DTU_sparse/model_1/rmvs00_L02}\end{overpic}
        \begin{overpic}[width=\figw\textwidth,trim={0cm 0cm 0cm 0cm},clip]{figures/results/compare/DTU_sparse/model_1/gipuma00_L02}\end{overpic}
        \captionof{subfigure}{\textit{Sparsity=5} }
    \end{minipage}
    \begin{minipage}[b]{\colw\textwidth}
        %includegraphics[width=\figw\textwidth,trim={0cm 0cm 0cm 0cm},clip]{figures/results/model13/camp}
        \begin{overpic}[width=\figw\textwidth,trim={0cm 0cm 0cm 0cm},clip]{figures/results/compare/DTU_sparse/model_1/surface+00_L03}\end{overpic}
        %\begin{overpic}[width=\figw\textwidth,trim={0cm 0cm 0cm 0cm},clip]{figures/results/model12/camp}\end{overpic}
        \begin{overpic}[width=\figw\textwidth,trim={0cm 0cm 0cm 0cm},clip]{figures/results/compare/DTU_sparse/model_1/rmvs00_L03}\end{overpic}
        \begin{overpic}[width=\figw\textwidth,trim={0cm 0cm 0cm 0cm},clip]{figures/results/compare/DTU_sparse/model_1/gipuma00_L03}\end{overpic}
        \captionof{subfigure}{\textit{Sparsity=7}}
    \end{minipage}
    \begin{minipage}[b]{\colw\textwidth}
        %includegraphics[width=\figw\textwidth,trim={0cm 0cm 0cm 0cm},clip]{figures/results/model13/tola}
        \begin{overpic}[width=\figw\textwidth,trim={0cm 0cm 0cm 0cm},clip]{figures/results/compare/DTU_sparse/model_1/surface+00_L04}\end{overpic}
        %\begin{overpic}[width=\figw\textwidth,trim={0cm 0cm 0cm 0cm},clip]{figures/results/model12/tola}\end{overpic}
        \begin{overpic}[width=\figw\textwidth,trim={0cm 0cm 0cm 0cm},clip]{figures/results/compare/DTU_sparse/model_1/rmvs00_L04}\end{overpic}
        \begin{overpic}[width=\figw\textwidth,trim={0cm 0cm 0cm 0cm},clip]{figures/results/compare/DTU_sparse/model_1/gipuma00_L04}\end{overpic}
        \captionof{subfigure}{\textit{Sparsity=9} }
    \end{minipage}
    \caption{    
        test  Qualitative comparison to the reference model from the DTU dataset \cite{aanaes2016large} and the reconstructions obtained by  \cite{campbell2008using,furu2010accurate,tola2012efficient,galliani2015massively}. 
        The rows show the models 9, 10, 11 from the DTU dataset \cite{aanaes2016large}. 
        %Because the proposed SurfaceNet learns the geometric knowledge of the local structure and infers structured surface, 
        %    such as the house roof in \textit{row 1} and the front / top side in \textit{row 3}.
    }
    \label{fig:DTU_sparse}
\end{figure*}

==> sections/fig/beta.tex <==

\begin{figure}[htbp]
    \centering
    \newcommand{\colw}{0.45}
    \newcommand{\figw}{1.0} % can bigger than 1
    \begin{subfigure}[b]{0.8\linewidth}
        \includegraphics[width=\figw\textwidth,trim={5cm 8cm 5.5cm 7cm},clip]{figures/table/beta}  %trim: l b r t
        % \caption{effect of $\beta$ when $\gamma=80\%$.}
    \end{subfigure}%

    % leave a blank line to change row       
    
    \begin{subfigure}[b]{\colw\linewidth}
        \includegraphics[width=\figw\textwidth,trim={0cm 3cm 0cm 3cm},clip]{figures/results/model9/beta/0} %trim={5cm 7cm 15cm 6cm},
        \captionsetup{labelformat=empty}
        \caption{$\beta = 0$}
    \end{subfigure}
    ~ 
    \begin{subfigure}[b]{\colw\linewidth}
        \includegraphics[width=\figw\textwidth,trim={0cm 3cm 0cm 3cm},clip]{figures/results/model9/beta/3}
        \captionsetup{labelformat=empty}
        \caption{$\beta = 3$}
    \end{subfigure}
    ~ 
    \begin{subfigure}[b]{\colw\linewidth}
        \includegraphics[width=\figw\textwidth,trim={0cm 3cm 0cm 3cm},clip]{figures/results/model9/beta/6}
        \captionsetup{labelformat=empty}
        \caption{$\beta = 6$}
    \end{subfigure}
    ~ 
    \begin{subfigure}[b]{\colw\linewidth}
        \includegraphics[width=\figw\textwidth,trim={0cm 3cm 0cm 3cm},clip]{figures/results/model9/beta/9}
        \captionsetup{labelformat=empty}
        \caption{$\beta = 9$}
    \end{subfigure}
    \caption{
    Quantitative and qualitative evaluation of $\beta$.
        %The $\beta$ values $3/6/9$ have the similiar performance.
        %It is determined only based on the preference between the accuracy and the completeness.
}
\label{fig:beta}
\end{figure}



==> sections/fig/iter.tex <==
\begin{figure}[htbp]
    \centering
    \newcommand{\colw}{0.45}
    \newcommand{\figw}{1.0} % can bigger than 1
    \begin{subfigure}[t]{\colw\linewidth}
        \includegraphics[width=\figw\textwidth,trim={1cm 5cm 10cm 8cm},clip]{{{figures/results/model9/iter/iter0}}}
        \caption{initialization}
    \end{subfigure}%
    ~ 
    \begin{subfigure}[t]{\colw\linewidth}
        \includegraphics[width=\figw\textwidth,trim={1cm 5cm 10cm 8cm},clip]{{{figures/results/model9/iter/iter1}}}
        \caption{iteration 1}
    \end{subfigure}
    ~ 
    \begin{subfigure}[t]{\colw\linewidth}
        \includegraphics[width=\figw\textwidth,trim={1cm 5cm 10cm 8cm},clip]{{{figures/results/model9/iter/iter4}}}
        \caption{iteration 4}
    \end{subfigure}
    \begin{subfigure}[t]{\colw\linewidth}
        \includegraphics[width=\figw\textwidth,trim={1cm 5cm 10cm 8cm},clip]{{{figures/results/model9/iter/iter8}}}
        \caption{iteration 8}
    \end{subfigure}%
    \caption{
        The adaptive threshold is estimated by an iterative algorithm.
        The algorithm converges within a few iterations.
        %As the iteration goes on, more floating noisy surface is filtered out.
    }
   \label{fig:iter}
\end{figure}



==> sections/fig/more.tex <==


\begin{figure*}[htbp]
    \centering
    \newcommand{\colw}{0.16}
    \newcommand{\figw}{1.0} % can bigger than 1
    \addtocounter{subfigure}{-4}
    \begin{minipage}[b]{\colw\textwidth}
        %\includegraphics[width=\figw\textwidth,trim={0cm 0cm 0cm 0cm},clip]{figures/results/model13/gt}
        \begin{overpic}[width=\figw\textwidth,trim={0cm 0cm 0cm 0cm},clip]{figures/results/model9/gt}\end{overpic}
        %\begin{overpic}[width=\figw\textwidth,trim={0cm 0cm 0cm 0cm},clip]{figures/results/model12/gt}\end{overpic}
        \begin{overpic}[width=\figw\textwidth,trim={0cm 0cm 0cm 0cm},clip]{figures/results/model10/gt}\end{overpic}
        \begin{overpic}[width=\figw\textwidth,trim={0cm 0cm 0cm 0cm},clip]{figures/results/model11/gt}\end{overpic}
        \captionof{subfigure}{reference model}
        % \label{fig:sub1}
    \end{minipage}
    \begin{minipage}[b]{\colw\textwidth}
        %includegraphics[width=\figw\textwidth,trim={0cm 0cm 0cm 0cm},clip]{figures/results/model13/ours}
        \begin{overpic}[width=\figw\textwidth,trim={0cm 0cm 0cm 0cm},clip]{figures/results/model9/ours}\end{overpic}
        %\begin{overpic}[width=\figw\textwidth,trim={0cm 0cm 0cm 0cm},clip]{figures/results/model12/ours}\end{overpic}
        \begin{overpic}[width=\figw\textwidth,trim={0cm 0cm 0cm 0cm},clip]{figures/results/model10/ours}\end{overpic}
        \begin{overpic}[width=\figw\textwidth,trim={0cm 0cm 0cm 0cm},clip]{figures/results/model11/ours}\end{overpic}
        \captionof{subfigure}{\textbf{SurfaceNet}}
    \end{minipage}
    \begin{minipage}[b]{\colw\textwidth}
        %includegraphics[width=\figw\textwidth,trim={0cm 0cm 0cm 0cm},clip]{figures/results/model13/furu}
        \begin{overpic}[width=\figw\textwidth,trim={0cm 0cm 0cm 0cm},clip]{figures/results/model9/furu}\end{overpic}
        %\begin{overpic}[width=\figw\textwidth,trim={0cm 0cm 0cm 0cm},clip]{figures/results/model12/furu}\end{overpic}
        \begin{overpic}[width=\figw\textwidth,trim={0cm 0cm 0cm 0cm},clip]{figures/results/model10/furu}\end{overpic}
        \begin{overpic}[width=\figw\textwidth,trim={0cm 0cm 0cm 0cm},clip]{figures/results/model11/furu}\end{overpic}
        \captionof{subfigure}{\textit{camp} \cite{campbell2008using}}
    \end{minipage}
    \begin{minipage}[b]{\colw\textwidth}
        %includegraphics[width=\figw\textwidth,trim={0cm 0cm 0cm 0cm},clip]{figures/results/model13/camp}
        \begin{overpic}[width=\figw\textwidth,trim={0cm 0cm 0cm 0cm},clip]{figures/results/model9/camp}\end{overpic}
        %\begin{overpic}[width=\figw\textwidth,trim={0cm 0cm 0cm 0cm},clip]{figures/results/model12/camp}\end{overpic}
        \begin{overpic}[width=\figw\textwidth,trim={0cm 0cm 0cm 0cm},clip]{figures/results/model10/camp}\end{overpic}
        \begin{overpic}[width=\figw\textwidth,trim={0cm 0cm 0cm 0cm},clip]{figures/results/model11/camp}\end{overpic}
        \captionof{subfigure}{\textit{furu} \cite{furu2010accurate}}
    \end{minipage}
    \begin{minipage}[b]{\colw\textwidth}
        %includegraphics[width=\figw\textwidth,trim={0cm 0cm 0cm 0cm},clip]{figures/results/model13/tola}
        \begin{overpic}[width=\figw\textwidth,trim={0cm 0cm 0cm 0cm},clip]{figures/results/model9/tola}\end{overpic}
        %\begin{overpic}[width=\figw\textwidth,trim={0cm 0cm 0cm 0cm},clip]{figures/results/model12/tola}\end{overpic}
        \begin{overpic}[width=\figw\textwidth,trim={0cm 0cm 0cm 0cm},clip]{figures/results/model10/tola}\end{overpic}
        \begin{overpic}[width=\figw\textwidth,trim={0cm 0cm 0cm 0cm},clip]{figures/results/model11/tola}\end{overpic}
        \captionof{subfigure}{\textit{tola} \cite{tola2012efficient}}
    \end{minipage}
    \begin{minipage}[b]{\colw\textwidth}
        %includegraphics[width=\figw\textwidth,trim={0cm 0cm 0cm 0cm},clip]{figures/results/model13/gipuma}
        \begin{overpic}[width=\figw\textwidth,trim={0cm 0cm 0cm 0cm},clip]{figures/results/model9/gipuma}\end{overpic}
        %\begin{overpic}[width=\figw\textwidth,trim={0cm 0cm 0cm 0cm},clip]{figures/results/model12/gipuma}\end{overpic}
        \begin{overpic}[width=\figw\textwidth,trim={0cm 0cm 0cm 0cm},clip]{figures/results/model10/gipuma}\end{overpic}
        \begin{overpic}[width=\figw\textwidth,trim={0cm 0cm 0cm 0cm},clip]{figures/results/model11/gipuma}\end{overpic}
        % \begin{overpic}[width=\figw\textwidth]{figures/results/mesh-model2-gipuma}\end{overpic}
        \captionof{subfigure}{\textit{Gipuma} \cite{galliani2015massively}}
    \end{minipage}
    \caption{    
        Qualitative comparison to the reference model from the DTU dataset \cite{aanaes2016large} and the reconstructions obtained by  \cite{campbell2008using,furu2010accurate,tola2012efficient,galliani2015massively}. 
        The rows show the models 9, 10, 11 from the DTU dataset \cite{aanaes2016large}. 
        %Because the proposed SurfaceNet learns the geometric knowledge of the local structure and infers structured surface, 
        %    such as the house roof in \textit{row 1} and the front / top side in \textit{row 3}.
    }
    \label{fig:methods}
\end{figure*}




==> sections/fig/result_show_first.tex <==
\begin{figure}[t]
    \centering
    \newcommand{\colw}{0.3}
    \newcommand{\figw}{1.1} % can bigger than 1
    \begin{subfigure}[t]{\colw\linewidth}
        \includegraphics[width=\figw\textwidth,trim={2cm 0cm 0cm 0cm},clip]{figures/results/compare/DTU_sparse/model_23/surface+00_L00}
        % \includegraphics[width=\figw\textwidth]{{figures/results/rect_017_mean}.jpg}
        %\caption{}
    \end{subfigure}%
    ~ 
    \begin{subfigure}[t]{\colw\linewidth}
        \includegraphics[width=\figw\textwidth,trim={2cm 0cm 0cm 0cm},clip]{figures/results/compare/DTU_sparse/model_23/gipuma00_L02}
        %\caption{\textbf{}}
    \end{subfigure}
    ~ 
    \begin{subfigure}[t]{\colw\linewidth}
        \includegraphics[width=\figw\textwidth,trim={2cm 0cm 0cm 0cm},clip]{figures/results/compare/DTU_sparse/model_23/rmvs00_L02}
        %\caption{\textit{} \cite{campbell2008using}}
    \end{subfigure}
    ~ 
    \begin{subfigure}[t]{\colw\linewidth}
        \includegraphics[width=\figw\textwidth,trim={2cm 0cm 0cm 0cm},clip]{figures/results/compare/DTU_sparse/model_23/surface+00_L02}
        \caption{\textbf{SurfaceNet+}}
    \end{subfigure}
    ~ 
    \begin{subfigure}[t]{\colw\linewidth}
        \includegraphics[width=\figw\textwidth,trim={2cm 0cm 0cm 0cm},clip]{figures/results/compare/DTU_sparse/model_23/rmvs00_L03}
        \caption{\textit{R-MVSNet} }
    \end{subfigure}
    ~ 
    \begin{subfigure}[t]{\colw\linewidth}
        \includegraphics[width=\figw\textwidth,trim={2cm 0cm 0cm 0cm},clip]{figures/results/compare/DTU_sparse/model_23/gipuma00_L03}
        \caption{\textit{Gipuma} \cite{galliani2015massively}}
    \end{subfigure}%
    \caption{Sparse view reconstruction of the model $23$ of the DTU dataset \cite{aanaes2016large} in comparison to \cite{galliani2015massively}.
     Our end-to-end learning framework provides a relatively complete reconstruction.}
   \label{fig:showcase}
\end{figure}


==> sections/fig/table/score.tex <==
\begin{table*}[htbp]
\centering
\small
%\hspace{-0.5cm}

\begin{tabular}{c|c|ccc|ccc|ccc}
\hline
\multicolumn{1}{l}{\multirow{}{}{Sparsity}} & \multicolumn{1}{l|}{\multirow{}{}{Method}} & \multicolumn{3}{c|}{Mean Distance (mm)}                          & \multicolumn{3}{c|}{Percentage(\textless{}1mm)} & \multicolumn{3}{c}{Percentage(\textless{}2mm)} \\
\multicolumn{1}{l}{}                          & \multicolumn{1}{l|}{}                        & Acc   & \multicolumn{1}{l}{Comp} & \multicolumn{1}{l|}{Overall} & Percision        & Recall       & f-score       & Percision        & Recall       & f-score       \\ \hline
\multicolumn{1}{c|}{\multirow{}{}{1}}       & SurfaceNet+                                  & 0.345 & 0.946                     & \textbf{0.646}                       & 88.01               & 73.01           & \textbf{78.44}            & 92.33               & 78.10           & \textbf{83.55}            \\
\multicolumn{1}{c|}{}                         & R-MVSNet                                    & 0.343                      & 0.951                       & 0.647                       &  87.63               & 72.48           &77.09             & 91.74               & 76.39           & 82.01           \\
\multicolumn{1}{c|}{}                         & Gipuma                                      & 0.268                       &1.402                       & 0.835                       & 94.65               & 59.93          & 70.64            & 96.42               & 63.81           & 74.16            \\ \hline
\multicolumn{1}{c|}{\multirow{}{}{2}}       & SurfaceNet+                                 & 0.411                       & 0.911                        & \textbf{0.661}                     & 87.35                & 73.59             & \textbf{78.29}            & 91.73             & 78.08             & \textbf{83.21}            \\
\multicolumn{1}{c|}{}                         & R-MVSNet                                     & 0.434                       & 1.057                       & 0.746                        & 86.96               & 60.04           & 67.99           & 95.05               & 65.71         & 74.69            \\
\multicolumn{1}{c|}{}                         & Gipuma                                       &0.290                       & 1.738                      & 1.014                        & 94.66               & 55.14           & 67.00            & 96.84              & 60.87           & 72.18            \\ \hline
\multicolumn{1}{c|}{\multirow{}{}{3}}       & SurfaceNet+                                  & 0.414                       & 0.987                        & \textbf{0.701}                     & 86.06              & 74.41            & \textbf{78.15}            & 90.87              & 78.25            & \textbf{82.91}            \\
\multicolumn{1}{c|}{}                         & R-MVSNet                                     & 0.423                       & 1.628                       & 1.02                      & 89.55               & 48.03           & 59.28            & 96.96               & 57.92         & 69.04           \\
\multicolumn{1}{c|}{}                         & Gipuma                                       & 0.263                     & 2.073                     & 1.168                     & 95.51               & 50.88           & 64.63            & 9749              & 50.33           & 63.68            \\ \hline
\multicolumn{1}{c|}{\multirow{}{}{4}}       & SurfaceNet+                                   & 0.407                       & 0.994                        & \textbf{0.699}                         &    87.06              & 72.14           & \textbf{77.41}            & 91.36              & 77.15           & \textbf{82.57}            \\
\multicolumn{1}{c|}{}                         & R-MVSNet                                     & 0.413                       & 2.438                        & 1.426                       & 88.17               & 32.02           & 44.92            & 93.66              & 44.21           & 57.55            \\
\multicolumn{1}{c|}{}                         & Gipuma                                      & 0.444                      & 2.059                      & 1.252                         & 91.95               & 46.65          & 59.76            & 94.95              & 55.16          & 67.71            \\ \hline
\multicolumn{1}{c|}{\multirow{}{}{5}}       & SurfaceNet+                                   & 0.396                       & 1.002                        & \textbf{0.699}                          & 88.58               & 71.63           & \textbf{77.48}            &  92.86             & 76.04            & \textbf{82.28}           \\
\multicolumn{1}{c|}{}                         & R-MVSNet                                      & 0.387                       & 4.474                       & 2.431                          & 89.26               & 20.51           & 31.60            & 93.99              & 32.74          & 46.37            \\
\multicolumn{1}{c|}{}                         & Gipuma                                       & 0.418                     & 2.814                        & 1.616                            & 92.38               & 38.53           & 52.36            & 95.10               & 48.15           & 61.78           \\ \hline
\multicolumn{1}{c|}{\multirow{}{}{6}}       & SurfaceNet+                                   & 0.388                      & 1.109                      & \textbf{0.749}                         & 86.74            & 67.26          & \textbf{74.93}            & 92.05               & 72.19           & \textbf{80.64}            \\
\multicolumn{1}{c|}{}                         & R-MVSNet                                     & 0.384                       & 6.467                        & 3.426                           & 91.65               & 08.49          & 14.28            & 94.70              & 16.60          & 26.28           \\
\multicolumn{1}{c|}{}                         & Gipuma                                         & 0.422                     & 3.017                        & 1.719                          & 92.46               & 30.37           & 43.99            & 95.32               & 40.80           & 55.28            \\ \hline
\multicolumn{1}{c|}{\multirow{}{}{7}}       & SurfaceNet+                                   & 0.379                      & 1.053                      & \textbf{0.716}                         & 91.36              &   72.23        & \textbf{75.59}            & 95.21                &  76.54           & \textbf{81.86}             \\
\multicolumn{1}{c|}{}                         & R-MVSNet                                     & empty                      & empty                        & empty                           & empty              & empty          & empty           & empty              & empty           & empty            \\
\multicolumn{1}{c|}{}                         & Gipuma                                         & 0.531                     & 3.358                        & 1.945                           & 85.35               & 17.91           & 28.66            & 90.78               & 28.00           & 41.31            \\ \hline
\end{tabular}%
\captionof{table}{
Quantitative results of reconstruction quality on the DTU dataset using distance metric(lower is better) and percentage metric\cite{Knapitsch2017}(higher is better) with respectively 1\textit{mm} and 2\textit{mm} thresholds. 
} \label{tab:DTU_score}
\end{table*}

==> sections/fig/table/score2.tex <==
\begin{table*}[htbp]
\centering
\small
%\hspace{-0.5cm}
\begin{tabular}{c|ccc|ccc|ccc}
\hline
\multirow{}{}{Sparsity} & \multicolumn{3}{c|}{SurfaceNet+}                                                              & \multicolumn{3}{c|}{R-MVSNet}                                                                   & \multicolumn{3}{c}{Gipuma}                                                                \\ \cline{2-10} 
                          & \multicolumn{1}{l}{acc(mm)} & \multicolumn{1}{l}{comp(mm)} & \multicolumn{1}{l|}{overall(mm)} & \multicolumn{1}{l}{acc(mm)} & \multicolumn{1}{l}{comp(mm)} & \multicolumn{1}{l|}{overall(mm)} & \multicolumn{1}{l}{acc(mm)} & \multicolumn{1}{l}{comp(mm)} & \multicolumn{1}{l}{overall(mm)} \\ \hline
1                         & 0.345                      & 0.946                       & \textbf{0.646}                           & 0.343                      & 0.951                       & 0.647                            & 0.268                       &1.402                       & 0.835                         \\
2                         & 0.411                       & 0.911                        & \textbf{0.661}                            & 0.434                       & 1.05                       & 0.746                           &0.290                       & 1.738                      & 1.014                       \\
3                         & 0.414                       & 0.987                        & \textbf{0.701}                            & 0.423                       & 1.628                       & 1.02                           & 0.263                     & 2.073                     & 1.168                        \\
4                         & 0.407                       & 0.994                        & \textbf{0.699}                            & 0.413                       & 2.438                        & 1.426                            & 0.444                      & 2.059                      & 1.252                          \\
5                         & 0.396                       & 1.002                        & \textbf{0.699}                            & 0.387                       & 4.474                       & 2.431                           & 0.418                     & 2.814                        & 1.616                        \\
6                         & 0.379                      & 1.053                      & \textbf{0.716}                          & 0.385                       & 6.21                        & 3.297                           & 0.531                     & 3.358                        & 1.945                          \\
7                         & 0.403                       & 1.190                        & \textbf{0.796}                            & empty                       & empty                       & empty                            & 0.686                      & 5.299                        & 2.992                           \\ \hline
\end{tabular}%
%\hspace{0.3cm}
% put caption below the \end{tabular} to put the caption at the bottom
\captionof{table}{
Quantitative results of reconstruction quality on the DTU dataset using distance metric(lower is better).
} \label{tab:DTU_score}
\end{table*}

% Please add the following required packages to your document preamble:
% \usepackage{multirow}

% Please add the following required packages to your document preamble:
% \usepackage{multirow}



==> sections/fig/table/tanks_compare.tex <==
\begin{table*}[htbp]
% \hspace{0.2cm}
% \centering
% \raggedleft
    \begin{tabular}{cccccc} %{| p{5cm} | p{5cm} | p{5cm} |}
    \hline
 Model & method & Sparsity = 1 & Sparsity = 3 & Sparsity = 5 & Sparsity = 7 \\   
  
    \hline
     \multirow{Lighthouse}   
  & SurfaceNet+ & 0.0 & 0.0 & 0.0 & 0.0 \\
  & R-MVSNet & 0.0 & 0.0 & 0.0 & 0.0\\
  & PMVSNet & 0.0 & 0.0 & 0.0 & 0.0\\
   \hline
     \multirow{Train}   
  & SurfaceNet+ & 0.0 & 0.0 & 0.0 & 0.0 \\
  & R-MVSNet & 0.0 & 0.0 & 0.0 & 0.0\\
  & PMVSNet & 0.0 & 0.0 & 0.0 & 0.0\\
   \hline
     \multirow{M60}   
  & SurfaceNet+ & 0.0 & 0.0 & 0.0 & 0.0 \\
  & R-MVSNet & 0.0 & 0.0 & 0.0 & 0.0\\
  & PMVSNet & 0.0 & 0.0 & 0.0 & 0.0\\
   \hline
     \multirow{Panther}   
  & SurfaceNet+ & 0.0 & 0.0 & 0.0 & 0.0 \\
  & R-MVSNet & 0.0 & 0.0 & 0.0 & 0.0\\
  & PMVSNet & 0.0 & 0.0 & 0.0 & 0.0\\
   \hline
     \hline

     \multirow{Mean}   
  & SurfaceNet+ & 0.0 & 0.0 & 0.0 & 0.0 \\
  & R-MVSNet & 0.0 & 0.0 & 0.0 & 0.0\\
  & PMVSNet & 0.0 & 0.0 & 0.0 & 0.0\\
   \hline
  \hline

    \end{tabular}
\caption{Quantitative comparision for sparse scene on the Tanks and Temple dataset \cite{Knapitsch2017}. 
        %$\tau$ has consistent affection for accuracy and completeness.
        } 
 \label{table:3DCNN-tab}
\end{table*}



\begin{table}[htbp]
\centering
\small
%\hspace{-0.5cm}
\begin{tabular}{c | c c | c c c}
\hline

\textbf{Dataset} & 
\multicolumn{2}{ c| }{\textbf{mean cubic number}} &
\multicolumn{3}{ c }{\textbf{multiple}} 
\\ 
\cline{2-6}
& \textbf{with} & \textbf{without} &  \textbf{mean} & \textbf{max} &  \textbf{min}\\
\hline

DTU               & 12905 & 67432 & 5.225 & 7.707 & 4.692 \\ \hline
Tanks and Temples & 6267 & 110541 & 17.638 & 43.74 &9.876 \\ \hline
\caption{Efficiency comparision of proposed method and SurfaceNet. 
        %$\tau$ has consistent affection for accuracy and completeness.
        } 
\label{table:cub_num}
\end{tabular}
\end{table}

==> sections/fig/tau.tex <==

\begin{figure}[htbp]
    \centering
    \newcommand{\colw}{0.30}
    \newcommand{\figw}{1.1} % can bigger than 1
    \begin{subfigure}[b]{0.99\linewidth}
        \includegraphics[width=1.0\textwidth,trim={0.0cm 0.0cm 0.0cm 0.0cm},clip]{figures/table/scatter/tau_gamma}
        % \caption{effect of $\tau$ when $\gamma=0\%; 100\%$.}
    \end{subfigure}%

    % leave a blank line to change row       
    \begin{subfigure}[t]{0.03\linewidth}
        \rotatebox{90}{$\gamma=0\%$}
    \end{subfigure}%
    ~
    \begin{subfigure}[t]{\colw\linewidth}
        \includegraphics[width=\figw\textwidth]{{figures/results/model9/t0.5_rp0}.jpg}
        % \caption{$\tau=0.5$}
    \end{subfigure}%
    ~ 
    \begin{subfigure}[t]{\colw\linewidth}
        \includegraphics[width=\figw\textwidth]{{figures/results/model9/t0.7_rp0}.jpg}
        % \caption{$\tau=0.7$}
    \end{subfigure}
    ~ 
    \begin{subfigure}[t]{\colw\linewidth}
        \includegraphics[width=\figw\textwidth]{{figures/results/model9/t0.9_rp0}.jpg}
        % \caption{$\tau=0.9$}
    \end{subfigure}
    \begin{subfigure}[t]{0.03\linewidth}
        \rotatebox{90}{$\gamma=100\%$}
    \end{subfigure}%
    ~
    \begin{subfigure}[t]{\colw\linewidth}
        \includegraphics[width=\figw\textwidth,trim={8.3cm 6.5cm 15.5cm 7.2cm},clip]{{figures/results/model9/tau/t0.5_rp10}.jpg}
        \captionsetup{labelformat=empty}
        \caption{$\tau=0.5$}
    \end{subfigure}%
    ~ 
    \begin{subfigure}[t]{\colw\linewidth}
        \includegraphics[width=\figw\textwidth,trim={8.3cm 6.5cm 15.5cm 7.2cm},clip]{{figures/results/model9/tau/t0.7_rp10}.jpg}
        \captionsetup{labelformat=empty}
        \caption{$\tau=0.7$}
    \end{subfigure}
    ~ 
    \begin{subfigure}[t]{\colw\linewidth}
        \includegraphics[width=\figw\textwidth,trim={8.3cm 6.5cm 15.5cm 7.2cm},clip]{{figures/results/model9/tau/t0.9_rp10}.jpg}
        \captionsetup{labelformat=empty}
        \caption{$\tau=0.9$}
    \end{subfigure}
    \caption{Quantitative and qualitative evaluation of $\tau$ for two values of $\gamma$. 
        %$\tau$ has consistent affection for accuracy and completeness.
        } 
   \label{fig:tau}
\end{figure}


==> sections/fig/tau_gamma.tex <==


\begin{figure}[htbp]
    \centering
    \newcommand{\colw}{0.30}
    \newcommand{\figw}{1.1} % can bigger than 1
    \begin{subfigure}[b]{0.99\linewidth}
        \includegraphics[width=1.0\textwidth,trim={0.0cm 0.0cm 0.0cm 0.0cm},clip]{figures/table/scatter/tau_gamma}
        % \caption{effect of $\tau$ when $\gamma=0\%; 100\%$.}
    \end{subfigure}%

    % leave a blank line to change row       
    \begin{subfigure}[t]{0.03\linewidth}
        \begin{minipage}{\textwidth}
            \vspace*{0.1cm}
            \rotatebox{90}{$\tau=0.5$}
        \end{minipage}
    \end{subfigure}%plot image
    ~
    \begin{subfigure}[t]{\colw\linewidth}
        % \includegraphics[width=\figw\textwidth]{{{figures/results/model9/t0.5_rp0}}}
        \begin{minipage}{\textwidth}
            \vspace*{0.1cm}
            \includegraphics[width=1\linewidth, keepaspectratio=true,trim={0cm 2cm 0cm 0cm},clip]{{{figures/results/model9/tau_gamma/t0.5_rp0}}}   % {{{,}}} can eliminate the file extension
            \includegraphics[width=1\linewidth, keepaspectratio=true,trim={0cm 6cm 0cm 5cm},clip]{{{figures/results/model9/tau_gamma/sec-t0.5_rp0}}}
        \end{minipage}%
        % \caption{$\tau=0.5$}
    \end{subfigure}%
    ~ 
    \begin{subfigure}[t]{\colw\linewidth}
        \begin{minipage}{\textwidth}
            \vspace*{0.1cm}
            \includegraphics[width=1\linewidth, keepaspectratio=true,trim={0cm 2cm 0cm 0cm},clip]{{{figures/results/model9/tau_gamma/t0.5_rp5}}}
            \includegraphics[width=1\linewidth, keepaspectratio=true,trim={0cm 6cm 0cm 5cm},clip]{{{figures/results/model9/tau_gamma/sec-t0.5_rp5}}}
        \end{minipage}
        % \caption{$\tau=0.7$}
    \end{subfigure}
    ~ 
    \begin{subfigure}[t]{\colw\linewidth}
        \begin{minipage}{\textwidth}
            \vspace*{0.1cm}
            \includegraphics[width=1\linewidth, keepaspectratio=true,trim={0cm 2cm 0cm 0cm},clip]{{{figures/results/model9/tau_gamma/t0.5_rp10}}}
            \includegraphics[width=1\linewidth, keepaspectratio=true,trim={0cm 6cm 0cm 5cm},clip]{{{figures/results/model9/tau_gamma/sec-t0.5_rp10}}}
        \end{minipage}
        % \caption{$\tau=0.9$}
    \end{subfigure}

    \begin{subfigure}[b]{0.03\linewidth}
        \begin{minipage}{\textwidth}
            \vspace*{0.1cm}
            \rotatebox{90}{$\tau=0.7$}
        \end{minipage}
    \end{subfigure}%
    ~
    \begin{subfigure}[t]{\colw\linewidth}
        \begin{minipage}{\textwidth}
            \vspace*{0.1cm}
            \includegraphics[width=1\linewidth,  keepaspectratio=true,trim={0cm 2cm 0cm 0cm},clip]{{{figures/results/model9/tau_gamma/t0.7_rp0}}}
            \includegraphics[width=1\linewidth,  keepaspectratio=true,trim={0cm 6cm 0cm 5cm},clip]{{{figures/results/model9/tau_gamma/sec-t0.7_rp0}}}
        \end{minipage}
        % \caption{$\tau=0.5$}
    \end{subfigure}%
    ~ 
    \begin{subfigure}[t]{\colw\linewidth}
        \begin{minipage}{\textwidth}
            \vspace*{0.1cm}
            \includegraphics[width=1\linewidth,  keepaspectratio=true,trim={0cm 2cm 0cm 0cm},clip]{{{figures/results/model9/tau_gamma/t0.7_rp5}}}
            \includegraphics[width=1\linewidth,  keepaspectratio=true,trim={0cm 6cm 0cm 5cm},clip]{{{figures/results/model9/tau_gamma/sec-t0.7_rp5}}}
        \end{minipage}
        % \caption{$\tau=0.7$}
    \end{subfigure}
    ~ 
    \begin{subfigure}[t]{\colw\linewidth}
        \begin{minipage}{\textwidth}
            \vspace*{0.1cm}
            \includegraphics[width=1\linewidth,  keepaspectratio=true,trim={0cm 2cm 0cm 0cm},clip]{{{figures/results/model9/tau_gamma/t0.7_rp10}}}
            \includegraphics[width=1\linewidth,  keepaspectratio=true,trim={0cm 6cm 0cm 5cm},clip]{{{figures/results/model9/tau_gamma/sec-t0.7_rp10}}}
        \end{minipage}
        % \caption{$\tau=0.9$}
    \end{subfigure}

    \begin{subfigure}[b]{0.03\linewidth}
        \begin{minipage}{\textwidth}
            \vspace*{0.1cm}
            \rotatebox{90}{$\tau=0.9$}
        \end{minipage}
    \end{subfigure}%
    ~
    \begin{subfigure}[t]{\colw\linewidth}
        \begin{minipage}{\textwidth}
            \vspace*{0.1cm}
            \includegraphics[width=1\linewidth,  keepaspectratio=true,trim={0cm 2cm 0cm 0cm},clip]{{{figures/results/model9/tau_gamma/t0.9_rp0}}}
            \includegraphics[width=1\linewidth,  keepaspectratio=true,trim={0cm 6cm 0cm 5cm},clip]{{{figures/results/model9/tau_gamma/sec-t0.9_rp0}}}
        \end{minipage}
        \captionsetup{labelformat=empty}
        \caption{$\gamma=0\%$}
    \end{subfigure}%
    ~ 
    \begin{subfigure}[t]{\colw\linewidth}
        \begin{minipage}{\textwidth}
            \vspace*{0.1cm}
            \includegraphics[width=1\linewidth,  keepaspectratio=true,trim={0cm 2cm 0cm 0cm},clip]{{{figures/results/model9/tau_gamma/t0.9_rp5}}}
            \includegraphics[width=1\linewidth,  keepaspectratio=true,trim={0cm 6cm 0cm 5cm},clip]{{{figures/results/model9/tau_gamma/sec-t0.9_rp5}}}
        \end{minipage}
        \captionsetup{labelformat=empty}
        \caption{$\gamma=50\%$}
    \end{subfigure}
    ~ 
    \begin{subfigure}[t]{\colw\linewidth}
        \begin{minipage}{\textwidth}
            \vspace*{0.1cm}
            \includegraphics[width=1\linewidth,  keepaspectratio=true,trim={0cm 2cm 0cm 0cm},clip]{{{figures/results/model9/tau_gamma/t0.9_rp10}}}
            \includegraphics[width=1\linewidth,  keepaspectratio=true,trim={0cm 6cm 0cm 5cm},clip]{{{figures/results/model9/tau_gamma/sec-t0.9_rp10}}}
        \end{minipage}
        \captionsetup{labelformat=empty}
        \caption{$\gamma=100\%$}
    \end{subfigure}
    \caption{Quantitative and qualitative evaluation of $\tau$ and $\gamma$. 
        %$\tau$ has consistent affection for accuracy and completeness.
        } 
   \label{fig:tau_gamma}
\end{figure}


==> sections/fig/view_selection.tex <==
\begin{figure}[htbp]
    \centering
    \newcommand{\colw}{0.48}
    \newcommand{\figw}{1.0} % can bigger than 1
    
     % leave a blank line to change row       
    \begin{subfigure}[b]{\colw\linewidth}
        \includegraphics[width=\figw\textwidth,trim={0cm 0cm 0cm 0cm},clip]{{{figures/method/view_selection/image_wise}}}
        \captionsetup{labelformat=empty}
        \caption{(a) image-wise}
    \end{subfigure}
    ~ 
    \begin{subfigure}[b]{\colw\linewidth}
        \includegraphics[width=\figw\textwidth,trim={0cm 0cm 0cm 0cm},clip]{{{figures/method/view_selection/pixel_wise}}}
        \captionsetup{labelformat=empty}
        \caption{(b) pixel-wise}
    \end{subfigure}
    ~ 
    \begin{subfigure}[b]{\colw\linewidth}
        \includegraphics[width=\figw\textwidth,trim={0cm 0cm 0cm 0cm},clip]{{{figures/method/view_selection/volume_wise}}}
        \captionsetup{labelformat=empty}
        \caption{(c) volume-wise}
    \end{subfigure}
    ~ 
    \begin{subfigure}[b]{\colw\linewidth}\label{subfigure:3d prior volume-wise}
        \includegraphics[width=\figw\textwidth,trim={0cm 0cm 0cm 0cm},clip]{{{figures/method/view_selection/3d_volume_wise}}}
        \captionsetup{labelformat=empty}
        \caption{(d) 3d prior volume-wise}
    \end{subfigure}
    \caption{Four different types of view selection and fusion method. We illustrate a 2D slice through the scene space and three camera views. The image patch selection and surface prediction are shown as forward and backward rays to and from each camera. The right and wrong geometry information are illustrated in blue and red respectively. (a) is image-wise view selection method, where patches from all views are selected and fused together after patch matching. (b) is pixel-wise view selection method that select the correct view pairs pixel by pixel but still fuses with wrong view information. (c) is volume-wise view selection which selects views and predicts results after picking high confidence views volume by volume. But it suffers from wrong view selection in self-occlusion area and similar pattern regions. %since it only use 2D image information for selection.%
    (d) is our proposed method which is an upgraded version of (c) that combine 3D geomretry prior to select the correct views.  }
    
% \ref{subfig:Nv1_weighted} to \ref{subfig:Nv6_weighted}
      
   \label{fig:view_selection_wise}
\end{figure}

==> sections/fig/volume_fusion.tex <==
\begin{figure}[htbp] % t/b/h: put the figure at the top / bottom / here
    \centering
    \includegraphics[width=0.8\linewidth]{figures/results/ablation/fusion_ablation} % scale=1 / width=0.8\linewidth\textwidth
    \caption{
    \words{Evaluation of the volumetric depth-map fusion method\cite{Zach2008}, which leads to comparable MVS results compared with the original depth-map fusion methods of Gipuma\cite{galliani2015massively} and R-MVSNet\cite{yao2019recurrent}.}}
    \label{fig:volume_fusion}
\end{figure}
